On Modular and Fully-Abstract Compilation -- Technical Appendix

Secure compilation studies compilers that generate target-level components that are as secure as their source-level counterparts. Full abstraction is the most widely-proven property when defining a secure compiler. A compiler is modular if it allows different components to be compiled independently and then to be linked together to form a whole program. Unfortunately, many existing fully-abstract compilers to untyped machine code are not modular. So, while fully-abstractly compiled components are secure from malicious attackers, if they are linked against each other the resulting component may become vulnerable to attacks. This paper studies how to devise modular, fully-abstract compilers. It first analyses the attacks arising when compiled programs are linked together, identifying security threats that are due to linking. Then, it defines a compiler from an object-based language with method calls and dynamic memory allocation to untyped assembly language extended with a memory isolation mechanism. The paper provides a proof sketch that the defined compiler is fully-abstract and modular, so its output can be linked together without introducing security violations.

==> bodies/aimtrsem.tex <==
% !TEX root = ./../scmp.tex

\subsection{Trace Equivalence for Securely-Compiled Components in \aim}\label{sec:aimtrsem}
This section defines a trace equivalence to reason about securely-compiled components in \aim.
Trace equivalence is a simpler tool to reason about equivalence of components than contextual equivalence~\cite{llfatr-j,scoo-j,abadiLayout,Jagadeesan,javaJr}.
Trace equivalence relates two components that exhibit the same trace semantics.
Trace semantics describes the behaviour of a component as a set of traces.
Traces are sequences of actions \trg{\OB{\alpha}} that obey to the following syntax.
\begin{align*}
&\mi{labels}& \trg{\lambda} ::=&\ \trg{\alpha}\mid\ \trg{\tau}
	&
&\mi{actions}& \trg{\alpha}\ ::=&\ \trg{\gamma!} \mid\ \trg{\gamma?} \mid\  \trg{\surd}
	\\
&\mi{observables}&	\trg{\gamma} ::=&\ \clgen{\ \trg{a}\ \trg{\OB{w}}} \mid\ \rtgen{\ \trg{a}\ \trg{w},\trg{w'}}
\end{align*}
Labels $\trg{\lambda}$ generated by the trace semantics can be actions $\trg{\alpha}$ or the silent action $\trg{\tau}$.
The silent action $\trg{\tau}$ is generated by unobservable transitions, thus these labels are not accumulated in traces.
Actions $\trg{\alpha}$ can be an observable, decorated action $\trg{\gamma}$ or a tick $\trg{\surd}$, which indicates termination of the computation.
Observable actions $\trg{\gamma}$ are either a function call to an address $\trg{a}$ with parameters \trg{\OB{w}}, or a return of value $\trg{w'}$ to address $\trg{a}$ by the module whose id is \trg{w}.
Decorations $\trg{?}$ or $\trg{!}$ indicate whether unprotected code performs the action ($\trg{?}$) or receives it ($\trg{!}$).

Define a component state with $\trg{\Theta}$, it indicates either that the execution is within a component or that the execution is in an unknown location.
Formally: $\trg{\Theta}::= (\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})\mid\blk$.
$\trg{\Theta_0}(\trg{P},\trg{h})$ denotes the initial state of a component $\trg{P}=(\trg{P},\trg{\OB{s}},\trg{t})$ with a nonce oracle $\trg{h}$.
Formally: $\trg{\Theta_0}(\trg{P},\trg{h})=\blk$.
Relation $\xtol{\trg{{\lambda}}}\ \subseteq\trg{\Theta}\times\trg{{\lambda}}\times\trg{\Theta}$ captures how single labels are generated.
The reflexive-transitive closure of $\xtol{\trg{{\lambda}}}$ accumulates labels in traces and filters out silent traces; it is captured by relation $\Xtol{\trg{\OB{\alpha}}}\ \subseteq\trg{\Theta}\times\trg{\OB{\alpha}}\times\trg{\Theta}$. 
Patrignani and Clarke~\cite{llfatr-j} defined a trace semantics for a single-module version of \aim; its multi-module adaptation, tailored for the components generated by our compiler, is presented below. 
A notable addition is the recording of module id inserted by caller-callee authentication when \asm{ret} labels are generated.
The auxiliary functions adopted for the trace semantics are used to tell if an address is an entry point (\acp{methodEntryPoint}), or if it is the return entry point (\acp{returnEntryPoint}).
Additionally, function \acp{exitJump} detects jumps outside the memory space of a component; function \acp{stuck} tells if a state is stuck.
\begin{figure}
\centering
\small
	\typerule{Trace-call}{
		\trg{\OB{w}} = \trg{w_0},\cdots,\trg{w_k}
		&
		\trg{r}=[\asm{r_0}\mapsto\trg{w_0},\cdots,\asm{r_{5+k}}\mapsto\trg{w_{5+k}}]
		&
		\trg{\OB{s}}\vdash\acp{methodEntryPoint}(\trg{p})
		\\
		\src{m}:\src{t}(\src{t_1\cdots,t_k})\to\src{t}\mapsto\trg{p} \in \trg{\OB{EM}}
		&
		\trg{t} = \trg{\OB{EM}};\trg{\OB{EO}};\trg{\OB{RM}};\trg{\OB{RO}}
	}{
		\blk\xtol{\cl{\trg{p}\ \trg{\OB{w}}}}(\trg{p},\trg{r'},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
	}{trace-call}\quad 
	\typerule{Trace-outcall}{
		\trg{m}(\trg{p})= (\asm{jmp\ r_d\ r_i})
		&
		\trg{p'}=(\trg{\iota},\trg{\sigma})
		&
		\trg{r}(\asm{r_d})\mapsto\trg{\sigma}
		&
		\trg{r}(\asm{r_i})\mapsto\trg{\iota}
		\\
		\trg{\OB{w}} = \trg{w_0},\cdots,\trg{w_{5+k}}
		&
		\trg{r}=[\asm{r_0}\mapsto\trg{w_0},\cdots,\asm{r_{5+k}}\mapsto\trg{w_{5+k}}]
		&
		\trg{\OB{s}},\trg{t}\vdash\acp{exitJump}(\trg{p},\trg{p'})
		\\
		\trg{r}(\asm{r_4})\neq\trg{0}
		&
		\src{m}:\src{t}(\src{t_1\cdots,t_k})\to\src{t}\mapsto\trg{\iota};\trg{\sigma} \in \trg{\OB{RM}}
		&
		\trg{t} = \trg{\OB{EM}};\trg{\OB{EO}};\trg{\OB{RM}};\trg{\OB{RO}}
	}{
		(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})\xtol{\cb{\trg{p'}\ \trg{\OB{w}}}}\blk
	}{trace-outcall}\quad
	\typerule{Trace-returnback}{
		\trg{p}=(\trg{id},\trg{n})
		&
		\trg{r}=[\asm{r_3}\mapsto\trg{id'},\asm{r_5}\mapsto\trg{w'}]
		&
		\trg{\OB{s}}\vdash\acp{returnEntryPoint}(\trg{p})
	}{
		\blk\xtol{\rb{\trg{p}\ \trg{id'},\trg{w'}}}(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
	}{trace-retback}\quad
	\typerule{Eval-return}{
		\trg{m}(\trg{p})= (\asm{jmp\ r_d\ r_i})
		&
		\trg{p}=(\trg{id},\trg{n})
		&
		\trg{p'}=(\trg{id'},\trg{n'})
		&
		\trg{r}(\asm{r_d})\mapsto\trg{n'}
		&
		\trg{r}(\asm{r_i})\mapsto\trg{id'}
		\\
		\trg{r}=[\asm{r_5}\mapsto\trg{w'}]
		&
		\trg{\OB{s}},\trg{t}\vdash\acp{exitJump}(\trg{p},\trg{p'})
		&
		\trg{r}(\asm{r_4})\mapsto\trg{0}
	}{
		(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})\xtol{\rt{\trg{p'}\ \trg{id},\trg{w'}}} (\unk,\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
	}{trace-return}

	\hspace{-.5em}\typerule{Trace-termination}{
		%(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h})\tol(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'})
		\trg{\Theta}\tol\trg{\Theta'}
		\\
		\vdash\acp{stuck}(\trg{\Theta'})
		%(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'})
	}{
		\trg{\Theta}
		%(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
		\xtol{\trg{\surd}}
		\trg{\Theta'}
		%(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'},\trg{t})
	}{trace-tick}
	\typerule{Trace-tau}{
		\trg{\Theta}
		%(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h})
		\tol
		\trg{\Theta'}
		%(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'})
	}{
		\trg{\Theta}
		%(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
		\xtol{\trg{\tau}}
		\trg{\Theta'}
		%(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'},\trg{t})
	}{trace-tau}
	\typerule{Trace-refl}{
	}{
		\trg{\Theta}\Xtol{\epsilon}\trg{\Theta}
	}{trrefl}\ 
	\typerule{Trace-tau}{
		\trg{\Theta}\xtol{\trg{\tau}}\trg{\Theta'}
	}{
		\trg{\Theta}\Xtol{\epsilon}\trg{\Theta'}
	}{trtau}
	\typerule{Trace-trans}{
		%\trg{\Theta}\Xtol{\trg{\OB{\alpha}}}\trg{\Theta''} 
		\trg{\Theta}\xtol{\trg{{\alpha}}}\trg{\Theta''} 
		\\
		\trg{\Theta''}\Xtol{\trg{\OB{\alpha}'}}\trg{\Theta'}
	}{
		\trg{\Theta}\Xtol{\trg{\OB{\alpha}}\cdot\trg{\OB{\alpha}'}}\trg{\Theta'}
	}{trtrans}
	%\typerule{Trace-s-action}{
	%	\trg{\Theta}\xtol{\trg{\alpha}}\trg{\Theta'}
	%}{
	%	\trg{\Theta}\Xtol{\trg{\alpha}}\trg{\Theta'}
	%}{tract}
\end{figure}

Define the trace semantics of a component $\trg{P}$ as: $\taim{\trg{P}}=\{\trg{\OB{\alpha}} \mid \forall \trg{h}.\exists\trg{\Theta}.$ $\trg{\Theta_0}(\trg{P},\trg{h})\Xtol{\trg{\OB{\alpha}}}\trg{\Theta}\}$.
Two modules $\trg{P_1}$ and $\trg{P_2}$ are trace equivalent, denoted with $\trg{P_1}\teqaim\trg{P_2}$ if their trace semantics coincides.
\begin{definition}[Trace equivalence]\label{def:treqaim}
$\trg{P_1}\teqaim\trg{P_2}\triangleq$ $\taim{\trg{P_1}}=\taim{\trg{P_2}}$.
\end{definition}
For securely-compiled components, trace semantics coincides with contextual equivalence, as captured by \Cref{prop:fatracesaim}.
%\footnote{In this case, the trace semantics is said to be fully-abstract~\cite{javaJr,llfatr-j}.We do not use this terminology outside this section to avoid confusion when full-abstraction is related to a compilation scheme.	}
\begin{proposition}[Trace semantics coincides with contextual equivalence for securely compiled \jem components]\label{prop:fatracesaim}
$\forall \src{\mc{C}_1}, \src{\mc{C}_2}. \compaim{\src{\mc{C}_1}}\ceqaim \compaim{\src{\mc{C}_2}} \iff \compaim{\src{\mc{C}_1}}\teqaim \compaim{\src{\mc{C}_2}}$.
\end{proposition}
\begin{proofsketch}
This proof is analogous to the one for the single-module version of \aim~\cite{llfatr-j}.
Informally, we need to prove that labels capture all the information that is communicated between a securely-compiled component and external code.

Let us discuss \trg{!}-decorated actions first.
The assumption about \comp{\cdot} code ensures that all communication coming from a compiled component happen only via entry points.
Specifically, this communication is regulated by the code added via the \prot{\cdot} function.
In case of a \cb{\cdot} only the registers used to carry a parameter (including the current object) are passed because \fun{resetFlagsAndRegisters}{\cdot} ensures that other registers are always \trg{0}.
In case of a \rt{\cdot} \fun{resetFlagsAndRegisters}{\cdot} ensures that only the module \trg{id} and the returned value (in \asm{r_5}) are not always \trg{0}.

Concerning \trg{?}-decorated actions, nor the code inserted by \prot{\cdot} nor the one generated by \comp{\cdot} uses flags as set by external code, so flags are never used to convey information.
In case of a \cl{\cdot}, due to the assumption on the correctness of \comp{\cdot} and on the definition of \prot{\cdot} only the registers used to carry parameters are used for computation.
In case of a \rb{\cdot}, the only registers used for calculation by \prot{\cdot} are \asm{r_3} and \asm{r_5}, which are the only ones captured by the trace semantics.
\end{proofsketch}


==> bodies/algo-old.tex <==
Informally, the algorithm is used to build a \jem context that can distinguish two \jem components whose compiled counterparts are trace inequivalent.

The algorithm inputs two distinct \aim traces \trg{\OB{\alpha_1}} and \trg{\OB{\alpha_2}} and the two \jem components that generate them \src{\mc{C}_1} and \src{\mc{C}_2}.
In other words $\trg{\OB{\alpha_1}}\in\taim{\compaim{\src{\mc{C}_1}}}$ and $\trg{\OB{\alpha_2}}\in\taim{\compaim{\src{\mc{C}_2}}}$.
The algorithm outputs a single \jem component \src{\mc{C}} that is the context that can differentiate between \src{\mc{C}_1} and \src{\mc{C}_2}.
The two traces are the same up to the last action, therefore $\trg{\OB{\alpha_1}}\equiv\trg{\OB{\alpha}\alpha_1!}$ and $\trg{\OB{\alpha_2}}\equiv\trg{\OB{\alpha}\alpha_2!}$ where $\trg{\alpha_1!}\neq\trg{\alpha_2!}$.
Trace \trg{\OB{\alpha}} is called the \emph{common prefix} while the two actions $\trg{\alpha_1!}$ and $\trg{\alpha_2!}$ are the \emph{different actions}, which appear at index $i$.

Intuitively, the algorithm produces code \src{\mc{C}} that replicates all ?-decorated actions in the common prefix \trg{\OB{\alpha}}.
The !-decorated actions are made by the component that fills the hole of \src{\mc{C}} and the algorithm adds code to \src{\mc{C}} to update its internal state.
Then, \src{\mc{C}} performs the differentiation by terminating in case it detects \src{\mc{C}_1} and diverging in the other.

The algorithm is divided in three parts: building the skeleton (\skel{\src{\mc{C}_1},\src{\mc{C}_2}}), emulating the common prefix (\emul{\trg{\OB{\alpha}},\trg{t}}) and distinguishing the different actions (\diff{\trg{\alpha_1!},\trg{\alpha_2!},i}).
Following is an informal description of how the algorithm works, a complete formalisation can be found in the appendix.
\begin{description}
	\item[$\skel{\src{\mc{C}_1},\src{\mc{C}_2}}$] 
	returns a component whose \lstb{import} requirements are the classes defined in \src{\mc{C}_1} and \src{\mc{C}_2}.
	This component provides an implementation for the \lstb{import} requirements of \src{\mc{C}_1} and \src{\mc{C}_2}.
	This consists of classes with empty method stubs for all required class declarations and objects for all required object declarations.
	Finally, it contains helper classes that code generated in other parts of the algorithm will use.
	\src{\mc{C}_1} and \src{\mc{C}_2} are assumed to define the same classes and objects and require the same classes and objects; if this is not the case, they can be easily differentiated.
	\item[$\emul{\trg{\OB{\alpha}},\trg{t}}$]
	returns expressions that fill the method stubs created by \skel{\cdot} based on the different encountered instructions.
	Below is an informal description of what the \emul{\cdot} function must do in each case.
	!-decorated actions only update the meta-data used by the algorithm and of \src{\mc{C}}.
	There are cases in which a ?-decorated action cannot be emulated, for example a return when no method call was made, or a call to a method that expects a \src{\lstb{Bool}} and instead receives \trg{4} as parameter.
	These are actions that try to violate \jem abstractions; in this cases the algorithm must \fail\ and generate a differentiating component that does nothing.

	\begin{description}
		\item[$\cl{\trg{a}\ \trg{\OB{w}}}$] 
		In this case the produced code must call to method \src{m} compiled at address \trg{a}; \trg{t} tells which \aim addresses correspond to which \jem methods.
		Based on the (known) signature of \src{m}, the parameters \trg{\OB{w}} are emulated to their \jem counterpart.
		
		Primitively-typed parameters are emulated to their \jem counterpart, e.g., when a \src{\lstb{Bool}} is expected and \trg{0} is received, the parameter is emulated by \src{\lst{true}} because $\comp{\src{\lst{true}}}=\trg{0}$.
		Object-typed parameters are stored in globally-accessible tables based on the encoding of their type and of the id they have in \aim.
		These tables have getters and setters to retrieve objects based on their \aim id.
		
		\item[$\rb{\trg{a}\ \trg{w},\trg{w'}}$]
		In this case the produced code must return the value emulating \trg{w'}, as discussed in the call case.
		\item[$\cb{\trg{a}\ \trg{\OB{w}}}$ and $\rt{\trg{a}\ \trg{w},\trg{w'}}$]
		In these cases, the internal state of \src{\mc{C}} is updated.
		For example, \src{\mc{C}} keeps track of the index of the action that is emulating and of all allocated objects.
		In these cases, the index is incremented by 1 and all newly allocated objects received via \trg{\OB{w}} or \trg{w'} are added to the tables.
	\end{description}
	
	\item[$\diff{\trg{\alpha_1!},\trg{\alpha_2!},i}$]
	returns two different code fragments that will detect whether \src{\mc{C}} is interacting with \src{\mc{C}_1} or \src{\mc{C}_2}.
	Following is an overview of what the differentiating code must be based on the differences between the two actions.
	For space constraints, not all cases are presented.
	\begin{description}
		\item[different kind of actions] e.g., $\trg{\alpha_1!}=\cb{\ \trg{a}\ \trg{\OB{w}}}$ and $\trg{\alpha_2!} = \rt{\ \trg{a'}\ \trg{w},\trg{w'}}$.
		The differentiating code at this point terminates in the method of \trg{a} and diverges in the current method.
		\item[different primitive-typed returned value] e.g., $\trg{\alpha_1!}=\rt{\ \trg{a_1}\ \trg{w_1},\trg{w_1'}}$ and $\trg{\alpha_2!} = \rt{\ \trg{a_2}\ \trg{w_2},\trg{w_2'}}$.
		In this case the differentiating code is placed at the current method, it consists of a check whether the returned value is equal to the source-equivalent of \trg{w_1'}. 
		If so the code terminates, otherwise it diverges.
		\item[different method] e.g., $\trg{\alpha_1!}=\cb{\ \trg{a}\ \trg{\OB{w}}}$ and $\trg{\alpha_2!} = \cb{\ \trg{a'}\ \trg{\OB{w'}}}$.
		In this case the differentiating code is placed at the methods for \trg{a} and \trg{a'}.
		It terminates in the method for \trg{a} and it diverges in the other.
	\end{description}
\end{description}

==> bodies/bg.tex <==
% !TEX root = ./../scmp.tex
\section{Background Notions}\label{sec:bg}
This section describes \jem (\Cref{sec:informje}) and \aim (\Cref{sec:informaim}), respectively the source and the target language of the secure compiler.
Then it discusses the threat model that is considered in this paper (\Cref{sec:threatmodel}) and it formalises multi-principal full abstraction (\Cref{sec:informfaproof}).


\input{bodies/langs.tex}
\input{bodies/threat.tex}
\input{bodies/informfa}


==> bodies/extension.tex <==
% !TEX root = ./../scmp.tex

==> bodies/form.tex <==
% !TEX root = ./../scmp.tex
\section{Proving the Compilation Scheme Secure}\label{sec:form}
Firstly, this section describes how to account for randomisation in the definition of contextual equivalence for \aim (\Cref{sec:randomaim}).
Then, it presents trace semantics for \aim programs (\Cref{sec:traim}) and it proves that the compilation scheme of \Cref{sec:seccomp} is multi-principal fully abstract (\Cref{sec:proof}).




\subsection{Randomisation and Contextual Equivalence for \aim} \label{sec:randomaim}
To account for randomisation in \aim, a randomisation instruction must be added to the language, and the odds of guessing its outcome must be considered.

\aim includes \mtt{rand\ r_d} in the instruction set; its semantics is to initialise register \mtt{r_d} with a random value.
To model the semantics of \mtt{rand}, we use an \emph{oracles}~\cite{oracle}, which provide random values for the randomisation function.
Formally an oracle is an infinite stream values: $O::= v; O$.
Oracles affects \aim contexts \mb{P}, whose holes can now be filled by a pair consisting of a program and an oracle.

\Crefrange{ex:ceqora}{ex:ceqora2} describe the usage of oracles; \Cref{ex:ceqguess} discusses how guessing random numbers affects the definition of contextual equivalence.

\begin{example}[Obvious equivalences]\label{ex:ceqora}
With an explicit oracle, obvious equivalences are respected; a program $P_r$ that returns a random value is equivalent to itself.
\begin{lstlisting}[mathescape]
$\setcounter{line}{0}$$\assline{rand\ r_0}$		// call this program $P_r$
$\assline{ret}$						// return a random number in $\mtt{r_0}$
\end{lstlisting}
In fact, for any oracle $O$, there exists an oracle (the same oracle $O$) that makes the behaviour of $P_r$ independent of random values.

$P_r$ is also equivalent to the following snippet $P_{rr}$, which generates two random numbers and only returns the second.
\begin{lstlisting}[mathescape]
$\setcounter{line}{0}$$\assline{rand\ r_0}$		// generate a number
$\assline{rand\ r_0}$		// then generate a second number
$\assline{ret}$						// return the second random number in $\mtt{r_0}$
\end{lstlisting}
The oracle that must be used with $P_{rr}$ is one that has all elements of $O$ interleaved with other elements.
\end{example}
\begin{example}[Obvious inequivalences]\label{ex:ceqora2}
Consider a program that returns two random numbers and a program that returns the same random number twice.

\noindent\begin{minipage}{0.47\textwidth}
\begin{lstlisting}[mathescape]
$\setcounter{line}{100}$$\assline{rand\ r_0}$
$\assline{}$ $\cdots$ // copy $\mtt{r_0}$ in $\mtt{r_1}$
$\assline{ret}$	
\end{lstlisting}
\end{minipage}
\hspace{0.05\textwidth}
\begin{minipage}{0.47\textwidth}
\begin{lstlisting}[mathescape]
$\setcounter{line}{100}$$\assline{rand\ r_0}$
$\assline{}$$\mtt{\hl{rand\ r_1}}$
$\assline{ret}$	
\end{lstlisting}
\end{minipage}

For any oracle used with the left-hand side snippet, the oracle that contains the same value twice will make the right-hand side snippet equivalent to it.
However, there is no oracle that will make the opposite true.

Generalising these examples allows us to conclude that any two \aim programs are equivalent if for any oracle used with the first program, there exists an oracle for the second program such that they have the same behaviour \emph{and vice versa}.
\end{example}
\begin{example}[Guessing]\label{ex:ceqguess}
Consider two programs that store a random number (line 3) and then input from the external code on \mtt{r_1} (line 6).
If that input matches the random number, one returns 0, the other returns 1 (line 15), otherwise they both return 2 (line 14, the syntax is massaged for the sake of simplicity).

\noindent\begin{minipage}{0.47\textwidth}
\begin{lstlisting}[mathescape]
$\setcounter{line}{100}$$\assline{rand\ r_0}$
$\assline{movi\ r_1\ 120}$	// at address 120
$\assline{movs\ r_0\ r_1}$	// store $\mtt{r_0}$
$\assline{movi\ r_0\ 0}$	
// call unprotected code 	
$\assline{call\ r_0}$ $\cdots$	
$\assline{movi\ r_1\ 120}$		
// load the random number
$\assline{movl\ r_1\ r_5}$		
// compare it with argument $\mtt{r_1}$
$\assline{cmp~\ r_1\ r_5}$		
$\assline{movi\ r_3\ 111}$		
$\assline{je~~\ r_3}$			// if it is not zero
$\assline{ret~ 2}$				// return 2
$\assline{ret~ 1}$				// otherwise return 1
\end{lstlisting}
\end{minipage}
\hspace{0.05\textwidth}
\begin{minipage}{0.47\textwidth}
\begin{lstlisting}[mathescape]
$\setcounter{line}{100}$$\assline{rand\ r_0}$
$\assline{movi\ r_1\ 120}$	// at address 120
$\assline{movs\ r_0\ r_1}$	// store $\mtt{r_0}$
$\assline{movi\ r_0\ 0}$	
// call unprotected code 	
$\assline{call\ r_0}$ $\cdots$	
$\assline{movi\ r_1\ 120}$		
// load the random number
$\assline{movl\ r_1\ r_5}$		
// compare it with argument $\mtt{r_1}$
$\assline{cmp~\ r_1\ r_5}$		
$\assline{movi\ r_3\ }$		
$\assline{je~~\ r_3}$			// if it is not zero
$\assline{ret~ 2}$				// return 2
$\assline{ret}$ $\hl{0}$				// otherwise return 0
\end{lstlisting}
\end{minipage}

If the random function is strong enough, external world has very little chance of telling these programs apart; intuitively, that chance is $\sim\!\!1/2^\ell$ times the number of guesses.
However, the contexts considered in the definition of contextual equivalence are universally quantified.
Thus there is also a context that differentiates between the two programs by guessing the number.
The definition of contextual equivalence needs to incorporate probability concepts.
\end{example}

The probabilistic notion of contextual equivalence states that two programs are equivalent if they behave the same to a certain probability.
Denote the probability of a certain event with $\probf{\cdot}$ and let $\sigma$ range over the 0..1 interval.
\begin{definition}[Contextual preorder for \aim]\label{def:preaim}
$P_1\preqaims P_2 \triangleq$ $\probf{\forall \mb{P},~O_1,~\exists O_2.~\mb{P}[P_1,O_1]\divr\iff\mb{P}[P_2,O_2]\divr} > \sigma$.
\end{definition}
Contextual equivalence for \aim programs is thus defined as following.
\begin{definition}[Contextual equivalence for \aim]\label{def:ceqaim}
$P_1\ceqaims P_2 \triangleq P_1\preqaims P_2 $ and $ P_2\preqaims P_1$.
\end{definition}
For securely-compiled components, if the randomisation function has a guessability of $\sigma_g$, $\sigma$ must be $1-\sigma_g$.
Unprotected code can in fact only guess once, if the guess is wrong, a fault is detected and the execution is halted, therefore $\sigma$ accounts only for one guess.







\subsection{Trace Semantics for \aim}\label{sec:traim}
The trace semantics of \aim programs extends that of \ai programs (\ai is the single-module version of \aim) to account for multiple modules~\cite{llfatr}.

To reason about partial \aim programs (i.e., the securely compiled ones), use trace equivalence of \aim programs.
Trace equivalence relates two programs that exhibit the same trace semantics.
Trace semantics describes the behaviour of a program as sets of traces.
Traces are sequences of actions \OB{\alpha} that obey to the following syntax.
\begin{align*}
\lambda ::=&\ \alpha
	&\alpha ::=&\ \gamma \delta
		&\gamma ::=&\ \mtt{call}\ a\ \OB{v}
			&\delta ::=&\ ?
				\\
\mid&\ \tau
	&\mid&\  \surd
		&\mid&\ \mtt{ret}\ a\ v
			&\mid&\ !
\end{align*}
Labels $\lambda$ generated by the trace semantics can be actions $\alpha$ or the silent action $\tau$.
The silent action $\tau$ is generated by unobservable transitions, thus these labels are not accumulated in traces.
Actions $\alpha$ can be an observable, decorated action $\gamma\delta$ or of a tick $\surd$, which indicates termination of the computation.
Observable actions $\gamma$ represent either a function call to a certain address $a$ with a set of parameters \OB{v}, or a return of value $v$ to an address $a$.
Decorations $?$ or $!$ indicate whether unprotected code performs the action ($?$) or receives it ($!$).

Informally, a call ($\mtt{call}\ a\ \OB{v}?$) is generated for each jump to an entry point besides for a jump to the returnback entry point.
A jump to the returnback entry point in fact generates a return ($\mtt{ret}\ a\ v?$).
An outcall ($\mtt{call}\ a\ \OB{v}!$) is generated whenever a call instruction from the partial program jumps outside the partial program.
A returnback ($\mtt{ret}\ a\ v!$)  is the execution of a return instruction from the partial program that jumps outside the partial program.
Finally, the tick $\surd$ is generated when the execution is halted.

\begin{example}[Traces of example \aim programs]\label{ex:tracesaim}
Consider only the program spanning from address 100 to 200 from \Cref{ex:pmacode}, consider the rest of the memory space to be undefined.
The following traces are valid descriptions of the behaviour of that program (use $\cdots$ to gloss over unimportant details):
\begin{align*}
T_1 =&\ \mtt{call}\ 100\ 12,10,\cdots?\ \mtt{ret}\ 4\ 2!
	\\
T_2=&\ \mtt{call}\ 100\ 5,0,\cdots?\ \mtt{call}\ 300\ \cdots!
	\\
T_3=&\ \mtt{ret}\ 106\ 0?\ \mtt{ret}\ 4\ 0!
\end{align*}
$T_1$ captures the behaviour of the code in case it is called with \mtt{r_0} greater than \mtt{r_1}.
$T_2$ captures the opposite.
$T_3$ captures the behaviour of the code after it has called code in the other protected module.
\end{example}

Define an \aim program with $P$ and a program state with $\Theta$; let $\Theta_0(P,O)$ denote the initial state of a program $P$ with an oracle $O$.
Let relation $\Xtol{\OB{\alpha}}\ \subseteq\Theta\times\OB{\alpha}\times\Theta$ capture how traces are generated.
Define the trace semantics of a program $P$ as: $\taim{P}=\myset{\OB{\alpha}}{\forall O.\exists\Theta.\Theta_0(P,O)\Xtol{\OB{\alpha}}\Theta}$.
Two programs $P_1$ and $P_2$ are trace equivalent, denoted with $P_1\teqaims P_2$ if their trace semantics coincides with a certain probability.
\begin{definition}[Trace equivalence for \aim]\label{def:treqaim}
$P_1\teqaims P_2\triangleq  \probf{\taim{P_1,O_1}=\taim{P_2,O_2}} > \sigma$.
\end{definition}
For securely-compiled components, trace semantics coincides with contextual equivalence, as captured by \Cref{prop:fatracesaim}.\footnote{
		In this case, the trace semantics is said to be fully abstract~\cite{javaJr,llfatr,faSH}, we do not use this terminology outside this section to avoid confusion when full abstraction is related to compilation scheme.
	}
\begin{proposition}[Fully abstract trace semantics for securely compiled \jem programs]\label{prop:fatracesaim}
$\forall C_1, C_2, C^T \in \jem. \compaim{C_1+C^T}\ceqaims \compaim{C_2+C^T} \iff \compaim{C_1+C^T}\teqaims \compaim{C_2+C^T}$.
\end{proposition}
\begin{proofsketch}
Securely-compiled components only use \mtt{call} and \mtt{ret} instructions to jump outside protected code.
No other instruction is executed on external code, e.g., no reading or writing in unprotected memory.
Moreover, external code also can only jump to the entry points of protected code and it cannot perform any other instruction on protected code.
Since unused registers and flags are reset at each jump from and to the protected code, the information communicated on the labels captures the behaviour of protected code precisely.
\end{proofsketch}


\input{./bodies/proof}


==> bodies/hlcomp.tex <==
% !TEX root = ./../scmp.tex

\subsection{The Secure Compiler, Informally}\label{sec:hlcomp}
Before presenting the details of \compaim{\cdot}, this section gives an informal description of the structure and the behaviour of \compaim{\cdot}. % (\Cref{fig:idea}).
Let us first analyse all possible interactions that can happen between (not-yet-securely)-compiled code \trg{M} and external code \trg{\mb{P}} at the \aim level (\Cref{fig:interactions}).
\myfig{\centering\small
\tikzpic{\small
	\node[] (c1){\trg{\mb{P}}};
	\node[right = of c1.east, xshift = 2em] (m1){\trg{M}};
	\draw[->] (c1.east) to node[above](ca1){\mtt{jump}} (m1.west);

	\node[below = of c1.north] (m3){\trg{M}};
	\node[right = of m3.east, xshift = 2em] (c3){\trg{\mb{P}}};
	\draw[->] (m3.east) to node[above](ca2){\mtt{jump}} (c3.west);
	
	\node[right = of m1.east, xshift = 2em] (c5){\trg{\mb{P}}};
	\node[right = of c5.east, xshift = 2em] (m5){\trg{M}};
	\draw[->] (c5.east) to node[above](rdwr1){\mtt{rd-wr}} (m5.west);
	
	\node[below = of c5.north] (m6){\trg{M}};
	\node[right = of m6.east, xshift = 2em] (c6){\trg{\mb{P}}};
	\draw[->] (m6.east) to node[above](rdwr2){\mtt{rd-wr}} (c6.west);

	\node[left = of c1.east] (n1){1)};
	\node[below = of n1.north] (n2){2)};
	\node[left = of c5.east] (n3){3)};
	\node[below = of n3.north] (n4){4)};

	\node[below = of n4.north, yshift = -0.5em] (n4b){};
}
}{interactions}{Possible assembly-level interactions: a jump towards a module (1), a jump from a module (2) a read/write to a module memory (3) a read/write from a module (4).}

Interaction 3 is prevented by \PMA while interaction 4 is prevented by the fact that only correct code executes and that kind of interaction is not allowed in \jem.

Let us now analyse the most relevant security-wise of the two remaining interactions: number 1.
From the \jem perspective of \aim code interaction 1 can be viewed in four cases (\Cref{fig:interactions2}).
\myfig{\centering\small
\tikzpic{
	\node[] (c1){\trg{\mb{P}}};
	\node[right = of c1.east, xshift = 4em] (m1){\trg{M}};
	\draw[->] (c1.east) to node[above](ca1){\mtt{call}} (m1.west);

	\node[below = of c1.north] (m3){\trg{\mb{P}}};
	\node[right = of m3.east, xshift = 4em] (c3){\trg{M}};
	\draw[->] (m3.east) to node[above](ca2){\mtt{return}} (c3.west);
	
	\node[right = of m1.east, xshift = 3em] (c5){\trg{\mb{P}}};
	\node[right = of c5.east, xshift = 4em] (m5){\trg{M}};
	\draw[->] (c5.east) to node[above](rdwr1){\mtt{call (bad)}} (m5.west);
	
	\node[below = of c5.north] (m6){\trg{\mb{P}}};
	\node[right = of m6.east, xshift = 4em] (c6){\trg{M}};
	\draw[->] (m6.east) to node[above](rdwr2){\mtt{return (bad)}} (c6.west);

	\node[left = of c1.east] (n1){1-a)};
	\node[below = of n1.north] (n2){1-b)};
	\node[left = of c5.east] (n3){1-c)};
	\node[below = of n3.north] (n4){1-d)};

	\node[below = of n4.north, yshift = -0.5em] (n4b){};
}
}{interactions2}{Possible kinds of jumps from \trg{\mb{P}} to \trg{M}: function calls and returns.}

Interaction 1 can only be a call (Case 1-a) or a return (Case 1-b) because method calls and returns are the only kind of interaction that can be done in \jem.
Both calls and returns can be normal or \emph{bad}.
Intuitively an bad interaction is one that generates a problem such as those presented in \Cref{sec:probs} (e.g., a bad return is one that causes call-stack shortcutting).

The goal of \compaim{\cdot}, and more specifically of \prot{\cdot} and \sys, is to prevent ill-formed communication (Cases 1 and 2 in \Cref{fig:idea}) and be transparent for well-formed ones (Case 0 in \Cref{fig:idea}).
\myfig{
\tikzpic{\small
	%\node[] (c1){\trg{\mb{P}}};
	%\node[right = of c1.east, xshift = 4em] (m1){\trg{M}};
	%\draw[->] (c1.east) to node[above](ca1){\mtt{jump}} (m1.west);


    %\draw[dashed] (-0.5,-0.5) -- (7.5,-0.5);
	
%	\node[below = of c1.north] (m3){\trg{M}};
%	\node[right = of m3.east, xshift = 2em] (c3){\trg{\mb{P}}};
%	\draw[->] (m3.east) to node[above](ca2){\mtt{jump}} (c3.west);
	
%	\node[below = of m3.north] (c5){\trg{\mb{P}}};
%	\node[right = of c5.east, xshift = 2em] (m5){\trg{M}};
%	\draw[->] (c5.east) to node[above](rdwr1){\mtt{rd-wr}} (m5.west);
	
%	\node[below = of c5.north] (m6){\trg{M}};
%	\node[right = of m6.east, xshift = 2em] (c6){\trg{\mb{P}}};
%	\draw[->] (m6.east) to node[above](rdwr2){\mtt{rd-wr}} (c6.west);

%	\node[left = of c1.east] (n1){1)};
%	\node[below = of n1.north] (n2){2)};
%	\node[below = of n2.north] (n3){3)};
%	\node[below = of n3.north] (n4){4)};

	
%	\node[below = of m6.south] (c1b){\trg{\mb{P}}};
	\node[] (c1b){\trg{\mb{P}}};
	\node[right = of c1b.east, xshift = 4em] (sys1){\sys};
	\draw[->] (c1b.east) to node[above](ca1b){\mtt{jump} (good)} (sys1.west);	
	\node[right = of sys1.east] (p1b){\prot{\trg{M}}};
	\draw[->] (sys1.east) to (p1b.west);	
	\node[right = of p1b.east] (m1b){\trg{M}};
	\draw[->] (p1b.east) to (m1b.west);	
	
	\node[below = of c1b.north] (c2b){\trg{\mb{P}}};
	\node[right = of c2b.east, xshift = 4em] (sys2){\sys};
	\draw[->] (c2b.east) to node[above](ca2b){\mtt{jump} (bad)} (sys2.west);	
	
	\node[below = of c2b.north] (c3b){\trg{\mb{P}}};
	\node[right = of c3b.east, xshift = 4em] (sys3){\sys};
	\draw[->] (c3b.east) to node[above](ca3b){\mtt{jump} (bad)} (sys3.west);	
	\node[right = of sys3.east] (p3b){\prot{\trg{M}}};
	\draw[->] (sys3.east) to (p3b.west);	

	\node[left = of c1b.east] (n1b){0)};
	
%	\node[below = of c1b.north] (m2b){\trg{M}};
%	\node[right = of m2b.east] (p2b){\prot{\trg{M}}};
%	\draw[->] (m2b.east) to (p2b.west);	
%	\node[right = of p2b.east] (sys2){\sys};
%	\draw[->] (p2b.east) to (sys2.west);	
%	\node[right = of sys2.east, xshift = 2em] (c2b){\trg{\mb{P}}};
%	\draw[->] (sys2.east) to node[above](ca2b){\mtt{jump}} (c2b.west);	

%	\node[left = of c1b.east] (n1b){1)};
	\node[below = of n1b.north] (n2b){1)};
	\node[below = of n2b.north] (n3b){2)};
%	\node[below = of n3b.north] (n4b){4)};
	\node[below = of c3b.north] (n4b){};
}
}{idea}{Visual behaviour of secure compiler additions.}





==> bodies/informfa.tex <==
% !TEX root = ./../scmp.tex
\subsection{Full Abstraction and Horizontal Compositionality}\label{sec:informfaproof}

Full-abstraction is the most widely-adopted notion for proving compiler security~\cite{AhmedFa,ahmedCPS,scoo-j,fstar2js,abadiLayout,Jagadeesan}.
As formalised by Abadi~\cite{abadiFa}, a compiler is fully-abstract if it preserves and reflects contextual equivalence of source and target components, as captured by \Cref{def:compfa} for a compiler \compgen{\cdot} from a source language \mc{S} to a target language \mc{T}.
\begin{definition}[Compiler full-abstraction]\label{def:compfa}
$\forall C_1, C_2 \in \mc{S}\ldotp C_1\ceq C_1 \iff \compgen{C_1}\ceq\compgen{C_2}$
\end{definition}
Contextual equivalence is the coarsest program equivalence and it can express a variety of program security properties such as confidentiality, integrity and so forth~\cite{scoo-j,abadiLayout,Jagadeesan}.
Its preservation and reflection therefore entails security.

One of the results of this paper is that \compaim{\cdot} is fully-abstract.
\begin{theorem}[\compaim{\cdot} is fully-abstract]
$\forall\src{\mc{C}_1},\src{\mc{C}_2},\src{\mc{C}_1}\ceqjem\src{\mc{C}_2}\iff\compaim{\src{\mc{C}_1}}\ceqaim\compaim{\src{\mc{C}_2}}$.
\end{theorem}

The proof of \Cref{thm:compaimisfa} is split in two cases: one for each direction of the co-implication.
\begin{description}
\item[$\forall\src{\mc{C}_1},\src{\mc{C}_2},\compaim{\src{\mc{C}_1}}\ceqaim\compaim{\src{\mc{C}_2}}\Rightarrow\src{\mc{C}_1}\ceqjem\src{\mc{C}_2}$]
	This direction is analogous to stating that \compaim{\cdot} outputs \aim programs that behave as the corresponding \jem programs.
	This is what most compilers achieve, at times even certifying the result~\cite{certComp,KRLMLa,related}; we are not interested in this direction.
	This direction can be proven assuming that the way \compaim{\cdot} translates \jem expressions is correct (a non-trivial assumption that is actively researched).

\item[$\forall\src{\mc{C}_1},\src{\mc{C}_2},\src{\mc{C}_1}\ceqjem\src{\mc{C}_2}\Rightarrow\compaim{\src{\mc{C}_1}}\ceqaim\compaim{\src{\mc{C}_2}}$]
	This direction states that \jem abstractions are preserved in the \aim output \compaim{\cdot} produces.
	Proving this direction requires reasoning about \aim contexts, which is difficult as they are low-level memories with no useful inductive structure.
	To avoid working with contexts, we replace the notion of contextual equivalence in \aim ($\ceqaim$) with that of trace equivalence in \aim ($\teqaim$, presented in \Cref{sec:aimtrsem}).
	%This provides us with an inductive principle to use in the proof.
	This direction is thus restated as $\forall\src{\mc{C}_1},\src{\mc{C}_2},\src{\mc{C}_1}\ceqjem\src{\mc{C}_2}\Rightarrow\compaim{\src{\mc{C}_1}}\teqaim\compaim{\src{\mc{C}_2}}$.
	The contrapositive of this statement is proven to hold: $\forall\src{\mc{C}_1},\src{\mc{C}_2},\compaim{\src{\mc{C}_1}}\nteqaim\compaim{\src{\mc{C}_2}}\Rightarrow\src{\mc{C}_1}\nceqjem\src{\mc{C}_2}$.

	So, assume two different traces of the compiled modules $\compaim{\src{\mc{C}_1}}$ and $\compaim{\src{\mc{C}_2}}$, where the first difference is an action generated by the modules.
	To prove $\src{\mc{C}_1}\nceqjem\src{\mc{C}_2}$ it suffices to show that \emph{there exists} a source-level context that behaves differently depending on whether its hole is filled with $\src{\mc{C}_1}$ or $\src{\mc{C}_2}$.
	Such a context is said to \emph{differentiate} $\src{\mc{C}_1}$ from $\src{\mc{C}_2}$.
	This established proof technique relies on an algorithm \algo{\cdot} that creates a \jem context (often called the \emph{witness}) that differentiates $\src{\mc{C}_1}$ from $\src{\mc{C}_2}$~\cite{faSemUML,scoo-j,llfatr-j}.
\end{description}

The novel result we are after for \compaim{\cdot} is modularity of our fully abstract compiler, i.e. components can be compiled separately and linked together afterwards without compromising security.
For this purpose, we indicate the linking of two \aim components as $\mylink{\trg{P_1},\trg{P_2}}$.
In this paper specifically, we want to be able to link any two \aim components \compaim{\src{\mc{C}_1}} and \compaim{\src{\mc{C}_2}} and be sure that $\mylink{\compaim{\src{\mc{C}_1}},\compaim{\src{\mc{C}_2}}}$ is still fully-abstract.
Formally, we will prove the theorem below as a corollary of \Cref{thm:compaimisfa}.
\begin{corollary}[Modular full-abstraction]
$\forall\src{\mc{C}_1},\src{\mc{C}_2},\src{\mc{C}}\ldotp \src{\mc{C}_1;C}\ceqjem\src{\mc{C}_2;C}\iff$ $\mylink{\compaim{\src{\mc{C}_1}},\compaim{\src{\mc{C}}}}\ceqaim\mylink{\compaim{\src{\mc{C}_2}},\compaim{\src{\mc{C}}}}$.
\end{corollary}


==> bodies/pmaprobs.tex <==
% !TEX root = ./../scmp.tex
\subsection{Secure Compiler Development}\label{sec:mistakes}
Following is the formal definition of the compiler \comp{\cdot}.
\begin{align*}
	\comp{\OB{\src{\OB{P_d^r}};\src{\OB{P_d^e}};\src{\OB{P_c}}}} &: \OB{(\trg{m_c}; \trg{m_d};\trg{t})}
	\\
	\comp{\OB{\src{\OB{P_d^r}};\src{\OB{P_d^e}};\src{\OB{P_c}}}} =&\ \OB{\comp{\src{\OB{P_c}_1}}+\cdots+\comp{\src{\OB{P_c}_n}}},	\trg{\mc{M}^r};\trg{\mc{O}^r};\trg{\mc{M}^e};\trg{\mc{O}^e}
		\\
		&\text{where } \trg{\mc{M}^r};\trg{\mc{O}^r}=\OB{\comp{\src{\OB{P_d^r}_1}}+\cdots+\comp{\src{\OB{P_d^r}_n}}}
		\\
		&\text{and }\trg{\mc{M}^e};\trg{\mc{O}^e}=\OB{\comp{\src{\OB{P_d^e}_1}}+\cdots+\comp{\src{\OB{P_d^e}_n}}}
	\\
	\comp{\src{{P_c}_1;\cdots;{P_c}_n}} =&\ \comp{\src{{P_c}_1}} \trg{+} \cdots \trg{+} \comp{\src{{P_c}_n}}
	\\
	\comp{\src{P_c}} &: (\trg{m_c};\trg{m_d})
	\\
	(\trg{m_c};\trg{_d}) \trg{+} (\trg{m_c'};\trg{m'_d}) =&\ (\trg{m_c+m_c'},\trg{m_d+m_d'}) 
		\\
		&\text{if }  \trg{m_c}\compat\trg{m_d}\compat\trg{m_c'}\compat\trg{m_d'}
	\\
	\comp{\src{{P_d}_1;\cdots;{P_d}_n}} =&\ \comp{\src{{P_d}_1}} + \cdots + \comp{\src{{P_d}_n}}
	\\
	\comp{\src{P_d}} &: \trg{\mc{M}};\trg{\mc{O}}
	\\
	\trg{\mc{M}_1};\trg{\mc{O}_1} +\cdots +\trg{\mc{M}_n};\trg{\mc{O}_n} =&\ \trg{\mc{M}_1}+\cdots+\trg{\mc{M}_n};\trg{\mc{O}_1}+\cdots+\trg{\mc{O}_n}
\end{align*}

Following is the formal definition of the compiler \compaim{\cdot}.
\begin{align*}
	\compaim{\src{\OB{C}}} =&\ \prot{\comp{\OB{\src{C}}}}
	\\
	\compaim{\src{\OB{\src{\OB{P_d^r}};\src{\OB{P_d^e}};\src{\OB{P_c}}}}} =&\ \prot{\comp{\OB{\src{\OB{P_d^r}};\src{\OB{P_d^e}};\src{\OB{P_c}}}}} 
\end{align*}

Following is the formal definition of the compiler \prot{\cdot}.
\begin{align*}
	\prot{(\trg{{m_c}_1}; \trg{{m_d}_1};\trg{t_1});\cdots;(\trg{{m_c}_n}; \trg{{m_d}_n};\trg{t_n})} =&\ \prot{\trg{{m_c}_1}; \trg{{m_d}_1};\trg{t_1}} \trg{+}\cdots
		\\
		&\ \trg{+} \prot{\trg{{m_c}_n}; \trg{{m_d}_n};\trg{t_n}}
\end{align*}
\begin{align*}
	\prot{\trg{m_c}; \trg{m_d};\trg{t}} :&\  (\trg{m};\trg{\OB{s}};\trg{t})
	\\
	(\trg{m};\trg{\OB{s}};\trg{t}) + (\trg{m'};\trg{\OB{s}'};\trg{t'}) =&\ (\trg{m}+\trg{m'};\trg{\OB{s}}+\trg{\OB{s}'};\trg{t}+\trg{t'})
		\\
		&\text{if } \trg{m}\compat\trg{m'} \text{ and } \trg{\OB{s}}\compat\trg{\OB{s}'}
	\\ 
	\trg{\mc{M}^r};\trg{\mc{O}^r};\trg{\mc{M}^e};\trg{\mc{O}^e} + \trg{{\mc{M}^r}'};\trg{{\mc{O}^r}'};\trg{{\mc{M}^e}'};\trg{{\mc{O}^e}'} :&\ \trg{\mc{M}^r};\trg{\mc{O}^r};\trg{\mc{M}^e};\trg{\mc{O}^e}
	\\ 
	\trg{\mc{M}^r};\trg{\mc{O}^r};\trg{\mc{M}^e};\trg{\mc{O}^e} + \trg{{\mc{M}^r}'};\trg{{\mc{O}^r}'};\trg{{\mc{M}^e}'};\trg{{\mc{O}^e}'} =&\ 
	\\
	\prot{\trg{m_c}; \trg{m_d};\trg{\mc{M}^r};\trg{\mc{O}^r};\trg{\mc{M}^e};\trg{\mc{O}^e}} =&\  \trg{m};\trg{s};\trg{{\mc{M}^r}'};\trg{{\mc{O}^r}'};\trg{{\mc{M}^e}'};\trg{{\mc{O}^e}'}
		\\
		&\text{where } \trg{s} =\ \fun{layoutOf}{\trg{\mc{M}^e}}
		\\
		&\text{and } \trg{m} =\ \biguplus_{\trg{a_i}\in\trg{\OB{a}}}\trg{m_{a_i}} + \trg{m_r} + \trg{m_t} + \trg{m_c} + \trg{m_{ce}} + \trg{m_d} + \trg{m_{de}}
		\\
		&\text{and } \trg{m_{a_i}} =\ \fun{methodEP}{\src{m},\src{M_t},\trg{a_m},\trg{a_i}}
		\\
		&\text{where } \trg{a_1},\cdots,\trg{a_n} = \fun{methodEPaddrs}{\trg{\OB{s}}}
		\\
		&\text{for all } \src{m}:\src{M_t}\mapsto\trg{a_m} \in \trg{\mc{M}^e}
		\\
		&\text{and } \trg{m_r} =\ \fun{returnbackEP}{\trg{a^r}}
		\\
		&\text{where } \trg{a^r} = \fun{returnbackEPaddr}{\trg{\OB{s}}}
		\\
		&\text{and } \trg{m_t} =\ \fun{throwEP}{\trg{a^t}}
		\\
		&\text{where } \trg{a^r} = \fun{throwEPaddr}{\trg{\OB{s}}}
		\\
		&\text{and } \trg{m_{ce}} =\ \trg{m_{tab}} + \fun{extraCode}{}
		\\
		&\text{and } \trg{m_{de}} =\ \fun{extraData}{}
		\\
		&\text{and } \trg{{\mc{M}^r}'} =\ \trg{{\mc{M}^r}}
		\\
		&\text{and } \trg{{\mc{O}^r}'} =\ \trg{{\mc{O}^r}}
		\\
		&\text{and } \trg{{\mc{M}^e}'} =\ \OB{\src{m_i}:\src{{M_t}_i}\mapsto\trg{a_i}}
		\\
		&\text{for all } \trg{a_i} \in \OB{\trg{a}}
		\\
		&\text{where } \src{m_i}:\src{{M_t}_i} = \trg{{\mc{M}^e}}(i)
		\\
		&\text{and } \trg{{\mc{O}^e}'} =\ \OB{\src{o_i}:\src{\OB{t}_i}\mapsto\trg{{a_o}_i}}
		\\
		&\text{for all } \trg{i}\in 1 .. \trg{n}
		\\
		&\text{where } \trg{{a_o}_i} = \trg{m_{tab}}(\trg{a_{base}}+\trg{i})
		\\
		&\text{where } \src{o_i}:\src{\OB{t}_i} = \trg{{\mc{O}^e}}(i)
		\\
		&\text{where } \trg{m_{tab}},\trg{n},\trg{a_{base}} = \fun{maskingTable}{\trg{\mc{O}^e}}
\end{align*}

==> bodies/prev.tex <==
% !TEX root = ./../scmp.tex
\subsection{The Base Compiler}\label{sec:previous}
Previous secure compilation works described how to securely compile the following language features: function calls, outcalls, dynamic memory allocation and exceptions~\cite{scoo-j}.

\myparagraph{Function calls} are calls from outside a module to inside it, they are implemented as jumps to the entry points of a module.
To securely compile function calls, a module must have an entry point for each method it exports.

\myparagraph{Outcalls} are function calls from within a module to outside of it -- essentially they are calls to the functions that the module requires from the code it links against to.
To securely compile outcalls, each module is given a secure stack where its code places allocation records for its functions.
The unprotected code is also given its own stack.
To allow returning from outcalls, an additional entry point must be added to entry points of a module.

Additional code at each entry point ensures that each parameter and the current object are values inhabiting the expected type.
These checks include primitive-typed value checks and dynamic typechecks on objects.
The former include checking that a value that is supposed to be of \src{\lstb{Unit}} type is \comp{\src{\lst{unit}}} and that a value that is supposed to be of \src{\lstb{Bool}} type is either \comp{\src{\lst{true}}} or \comp{\src{\lst{false}}}.
No checks are needed for values that are supposed to be of \src{\lstb{Int}} type as they can span the whole range of values expressible in a word.
Dynamic typechecks are made on all objects which are checked to have a type that conforms to the type that is expected for that parameter.
Object ids in \aim are addresses \trg{a} that point to where an object is located, the first word encodes the object's type; for modules this address points to the data section. \MP{ needs rewriting}


\myparagraph{Dynamic memory allocation}
is the creation of objects with the \lstb{new} instruction.
To securely compile dynamic memory allocation a \emph{masking table} must be added to the compiler output.
The masking table is indicated with \mc{O}, it is a map between target-level object ids and word-sized integers.
Before an object id is passed to external code, it is placed in the table, and the corresponding index is passed in place of the id; the same index must be passed whenever an already recorded object is passed.
This process is called \emph{masking}, thus the passed index is called the \emph{masking index}.
Since external code can only call functions on objects, object parameters at method entry point are expected to be masking indexes, which are used to retrieve the actual object id to be used in the computation.
At all entry points, if an object id of a type implemented in the protected code is retrieved, that object is checked to be of the expected type for the parameter it stands for.
Table \mc{O} is implemented as a word containing its length (\trg{a_{\mc{O}}}) followed by a list of target-level object ids \OB{\trg{a}}.
Retrieving index \trg{n} (denoted with $\mc{O}(\trg{n})$) is a failure if $\trg{n}>\trg{a}$, otherwise it results in the word located at address $\trg{a_{\mc{O}}+n}$.



\myparagraph{Exceptions} are errors that happen at runtime and that alter the flow of execution of a program.
To securely compile exceptions, an additional entry point is needed, called \emph{throw entry point}.
External code jumps to this entry point in order to throw an exception.
With exceptions, the interface types that an object implements are known, as some code can continuously throw an exception an catch at different interface types to know precisely the type of the exceptions.
This leads to a modification of the object id encoding that now needs an additional word that encodes all the interfaces that the object implements. \MP{ expand? make clearer?}

==> bodies/proofinform.tex <==
% !TEX root = ./../scmp.tex
\section{Full-Abstraction and Modularity of \compaim{\cdot}} \label{sec:proof}
As stated in \Cref{sec:intro}, a compiler is fully-abstract if it preserves and reflects contextual equivalence of source and target components.
This section presents how contextual equivalence is reflected (\Cref{sec:compcorrdir}) and preserved (\Cref{sec:compsecdir}) for \compaim{\cdot}.
Then it concludes by proving full-abstraction and modularity of \compaim{\cdot} (\Cref{sec:allproofs}).

All proofs are omitted and can be found in the appendix.








\subsection{\compaim{\cdot} Reflects Contextual Equivalence}\label{sec:compcorrdir}
Proving that \compaim{\cdot} reflects contextual equivalence (\Cref{thm:compaimcorr}) is analogous to proving that it is correct.
\begin{theorem}[\compaim{\cdot} preserves behaviour]\label{thm:compaimcorr}
$\forall\src{\mc{C}_1},\src{\mc{C}_2}.\compaim{\src{\mc{C}_1}}\ceqaim\compaim{\src{\mc{C}_2}}\Rightarrow\src{\mc{C}_1}\ceqjem\src{\mc{C}_2}$.
\end{theorem}

Intuitively, given \Cref{ass:comp-corr}, this holds because nor \prot{\cdot} nor the addition of \sys change the semantics of compiled programs.


















\subsection{\compaim{\cdot} Preserves Contextual Equivalence}\label{sec:compsecdir}
Proving that \compaim{\cdot} preserves contextual equivalence (\Cref{thm:compaimsecure}) is where we prove that \compaim{\cdot} is secure.
\Cref{thm:compaimsecure} intuitively states that \jem abstractions are preserved in the \aim output \compaim{\cdot} produces.
\begin{theorem}[\compaim{\cdot} is secure]\label{thm:compaimsecure} 
$\forall\src{\mc{C}_1},\src{\mc{C}_2}.\src{\mc{C}_1}\ceqjem\src{\mc{C}_2}\Rightarrow\compaim{\src{\mc{C}_1}}\ceqaim\compaim{\src{\mc{C}_2}}$.
\end{theorem}
To prove \Cref{thm:compaimsecure} we proceed as follows.
First, we devise a notion of trace equivalence $\teqaim$ for securely-compiled components (\Cref{sec:aimtrsem}).
$\teqaim$ is proven to be equivalent to $\ceqaim$, so the two notions can be exchanged (\Cref{thm:fatracesaim}).
Then we re-state the theorem in contrapositive form: 
	$$\forall\src{\mc{C}_1},\src{\mc{C}_2}.\compaim{\src{\mc{C}_1}}\nteqaim\compaim{\src{\mc{C}_2}}\Rightarrow\src{\mc{C}_1}\nceqjem\src{\mc{C}_2}$$
To prove that $\src{\mc{C}_1}\nceqjem\src{\mc{C}_2}$ we need to prove (by negating \Cref{def:ceqjem}) that there exist a context that, wlog, terminates with \src{\mc{C}_1} and diverges with \src{\mc{C}_2}.
This context is said to \emph{differentiate} between \src{\mc{C}_1} and \src{\mc{C}_2}.
Finally we devise an algorithm \algo{\cdot} that can distinguish between \jem components whose compiled counterparts are trace-inequivalent~\cite{faSemUML,scoo-j,llfatr-j} (\Cref{sec:algo}).
We prove that \algo{\cdot} is correct (\Cref{thm:algocorr}), so we can use it to prove that two \jem components are contextually-inequivalent if their compiled counterparts are trace-inequivalent.












\subsubsection{Trace Equivalence for Securely-Compiled Components in \aim}\label{sec:aimtrsem}
This section defines a trace equivalence to reason about securely-compiled components in \aim; it is inspired by the trace semantics for the single-module version of \aim~\cite{llfatr-j}.

Trace equivalence is a simpler tool to reason about equivalence of components than contextual equivalence~\cite{llfatr-j,scoo-j,abadiLayout,Jagadeesan,javaJr}.
Trace equivalence relates two components that exhibit the same trace semantics.
Trace semantics describes the behaviour of a component as a set of traces.
Traces are sequences of actions \trg{\OB{\alpha}} with the following syntax:
\begin{align*}
&\mi{labels}& \trg{\lambda} ::=&\ \trg{\alpha}\mid\ \trg{\tau}
	&
&\mi{actions}& \trg{\alpha}\ ::=&\ \trg{\gamma!} \mid\ \trg{\gamma?} \mid\  \trg{\surd}
\end{align*}\vspace{-2.3em}
\begin{align*}
&\mi{observables}&	\trg{\gamma} ::=&\ \clgen{\ \trg{a}\ \trg{\OB{w}}} \mid\ \rtgen{\ \trg{a}\ \trg{w},\trg{id}}
\end{align*}
Labels $\trg{\lambda}$ generated by the trace semantics can be actions $\trg{\alpha}$ or the silent action $\trg{\tau}$.
The silent action $\trg{\tau}$ is generated by unobservable transitions, thus these labels are not accumulated in traces.
Actions $\trg{\alpha}$ can be an observable, decorated action $\trg{\gamma}$ or a tick $\trg{\surd}$, which indicates termination of the computation.
Observable actions $\trg{\gamma}$ are either a function call to an address $\trg{a}$ with parameters \trg{\OB{w}}, or a return of value $\trg{w}$ to address $\trg{a}$ from the module with id \trg{id}.
Decorations $\trg{?}$ or $\trg{!}$ indicate whether unprotected code performs the action ($\trg{?}$) or receives it ($\trg{!}$).

Define a (compiled) component state with $\trg{\Theta}$, it indicates either that the execution is within a component or that the execution is in an unknown location.
Formally: $\trg{\Theta}::= (\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})\mid\blk$.
$\trg{\Theta_0}(\trg{P},\trg{h})$ denotes the initial state of a component $\trg{P}=(\trg{m},\trg{\OB{s}},\trg{t})$ with a nonce oracle $\trg{h}$.
Formally: $\trg{\Theta_0}(\trg{P},\trg{h})=\blk$.
Relation $\xtol{\trg{{\lambda}}}\ \subseteq\trg{\Theta}\times\trg{{\lambda}}\times\trg{\Theta}$ captures how single labels are generated.
The reflexive-transitive closure of $\xtol{\trg{{\lambda}}}$ accumulates labels in traces and filters out silent traces; it is captured by relation $\Xtol{\trg{\OB{\alpha}}}\ \subseteq\trg{\Theta}\times\trg{\OB{\alpha}}\times\trg{\Theta}$. 
The auxiliary functions adopted for the trace semantics are used to tell if an address is an entry point (\acp{methodEntryPoint}), or if it is the entry point related to the \fun{forwardReturn}{\cdot} procedure in \sys (\acp{forwardReturnEP}).
Function \acp{exitJump} detects jumps outside the memory space of a component; function \acp{stuck} tells if a state is stuck.
\begin{figure}
\centering
\small
	\typerule{Trace-call}{
		\trg{\OB{w}} = \trg{w_0},\cdots,\trg{w_k}
		&
		\trg{r}=[\asm{r_0}\mapsto\trg{w_0},\cdots,\asm{r_{6+k}}\mapsto\trg{w_{6+k}}]
		\\
		\trg{\OB{s}}\vdash\acp{methodEntryPoint}(\trg{p})
		&
		\src{m}:\src{t}(\src{t_1\cdots,t_k})\to\src{t}\mapsto\trg{p} \in \trg{\OB{EM}}
		\\
		\trg{t} = \trg{\OB{EM}};\trg{\OB{EO}};\trg{\OB{RM}};\trg{\OB{RO}}
	}{
		\blk\xtol{\cl{\trg{p}\ \trg{\OB{w}}}}(\trg{p},\trg{r'},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
	}{trace-call}\quad 
	\typerule{Trace-outcall}{
		\trg{m}(\trg{p})= (\asm{jmp\ r_d\ r_i})
		&
		\trg{p'}=(\trg{\iota},\trg{\sigma})
		&
		\trg{r}(\asm{r_d})\mapsto\trg{\sigma}
		&
		\trg{r}(\asm{r_i})\mapsto\trg{\iota}
		\\
		\trg{\OB{w}} = \trg{w_0},\cdots,\trg{w_{6+k}}
		&
		\trg{r}=[\asm{r_0}\mapsto\trg{w_0},\cdots,\asm{r_{6+k}}\mapsto\trg{w_{6+k}}]
		\\
		\trg{\OB{s}},\trg{t}\vdash\acp{exitJump}(\trg{p},\trg{p'})
		&
		\trg{r}(\asm{r_5})=\trg{3*\mc{N}_w}
		\\
		\src{m}:\src{t}(\src{t_1\cdots,t_k})\to\src{t}\mapsto\trg{\iota};\trg{\sigma} \in \trg{\OB{RM}}
		&
		\trg{t} = \trg{\OB{EM}};\trg{\OB{EO}};\trg{\OB{RM}};\trg{\OB{RO}}
	}{
		(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})\xtol{\cb{\trg{p'}\ \trg{\OB{w}}}}\blk
	}{trace-outcall}\quad
	\typerule{Trace-returnback}{
		%\trg{p}=(\trg{id},\trg{n})
		&
		\trg{r}=[\asm{r_0}\mapsto\trg{id'},\asm{r_6}\mapsto\trg{w}]
		&
		\trg{\OB{s}}\vdash\acp{forwardReturnEP}(\trg{p})
	}{
		\blk\xtol{\rb{\trg{p}\ \trg{w},\trg{id'}}}(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
	}{trace-retback}\quad
	\typerule{Eval-return}{
		\trg{m}(\trg{p})= (\asm{jmp\ r_d\ r_i})
		&
		\trg{p}=(\trg{id},\trg{n})
		&
		\trg{p'}=(\trg{id'},\trg{n'})
		\\
		\trg{r}(\asm{r_d})\mapsto\trg{n'}
		&
		\trg{r}(\asm{r_i})\mapsto\trg{id'}
		&
		\trg{r}=[\asm{r_6}\mapsto\trg{w}]
		\\
		\trg{\OB{s}},\trg{t}\vdash\acp{exitJump}(\trg{p},\trg{p'})
		&
		\trg{r}(\asm{r_5})\mapsto\trg{0}
	}{
		(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})\xtol{\rt{\trg{p'}\ \trg{w},\trg{id}}} (\unk,\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
	}{trace-return}

	\typerule{Trace-tau}{
		\trg{\Theta}
		%(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h})
		\tol
		\trg{\Theta'}
		%(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'})
	}{
		\trg{\Theta}
		%(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
		\xtol{\trg{\tau}}
		\trg{\Theta'}
		%(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'},\trg{t})
	}{trace-tau}
	\typerule{Trace-refl}{
	}{
		\trg{\Theta}\Xtol{\epsilon}\trg{\Theta}
	}{trrefl}
	\typerule{Trace-tau}{
		\trg{\Theta}\xtol{\trg{\tau}}\trg{\Theta'}
	}{
		\trg{\Theta}\Xtol{\epsilon}\trg{\Theta'}
	}{trtau}
	\typerule{Trace-trans}{
		%\trg{\Theta}\Xtol{\trg{\OB{\alpha}}}\trg{\Theta''} 
		\trg{\Theta}\xtol{\trg{{\alpha}}}\trg{\Theta''} 
		\\
		\trg{\Theta''}\Xtol{\trg{\OB{\alpha}'}}\trg{\Theta'}
	}{
		\trg{\Theta}\Xtol{\trg{\OB{\alpha}}\cdot\trg{\OB{\alpha}'}}\trg{\Theta'}
	}{trtrans}
	\typerule{Trace-termination}{
		%(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h})\tol(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'})
		\trg{\Theta}\tol\trg{\Theta'}
		\\
		\vdash\acp{stuck}(\trg{\Theta'})
		%(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'})
	}{
		\trg{\Theta}
		%(\trg{p},\trg{r},\trg{f},\trg{m},\trg{\OB{s}},\trg{h},\trg{t})
		\xtol{\trg{\surd}}
		\trg{\Theta'}
		%(\trg{p'},\trg{r'},\trg{f'},\trg{m'},\trg{\OB{s}},\trg{h'},\trg{t})
	}{trace-tick}
	%\typerule{Trace-s-action}{
	%	\trg{\Theta}\xtol{\trg{\alpha}}\trg{\Theta'}
	%}{
	%	\trg{\Theta}\Xtol{\trg{\alpha}}\trg{\Theta'}
	%}{tract}
\end{figure}

Define the trace semantics of a component $\trg{P}$ as: $\taim{\trg{P}}=\{\trg{\OB{\alpha}} \mid \forall \trg{h}.\exists\trg{\Theta}.$ $\trg{\Theta_0}(\trg{P},\trg{h})\Xtol{\trg{\OB{\alpha}}}\trg{\Theta}\}$.
Two modules $\trg{P_1}$ and $\trg{P_2}$ are trace equivalent, denoted with $\trg{P_1}\teqaim\trg{P_2}$ if their trace semantics coincides.
\begin{definition}[Trace equivalence]\label{def:treqaim}
$\trg{P_1}\teqaim\trg{P_2}\triangleq$ $\taim{\trg{P_1}}=\taim{\trg{P_2}}$.
\end{definition}
For securely-compiled components, trace semantics coincides with contextual equivalence (\Cref{thm:fatracesaim}).
\begin{theorem}[Trace semantics coincides with contextual equivalence for securely compiled \jem components]\label{thm:fatracesaim}
$\forall \src{\mc{C}_1}, \src{\mc{C}_2}. \compaim{\src{\mc{C}_1}}\ceqaim \compaim{\src{\mc{C}_2}} \iff \compaim{\src{\mc{C}_1}}\teqaim \compaim{\src{\mc{C}_2}}$.
\end{theorem}






















\subsubsection{Trace Back-Translation Algorithm \algo{\cdot}}\label{sec:algo}
Informally, the algorithm is used to build a \jem context that can distinguish two \jem components whose compiled counterparts are trace inequivalent.

The algorithm inputs two distinct \aim traces \trg{\OB{\alpha_1}} and \trg{\OB{\alpha_2}} and the two \jem components that generate them \src{\mc{C}_1} and \src{\mc{C}_2}.
In other words $\trg{\OB{\alpha_1}}\in\taim{\compaim{\src{\mc{C}_1}}}$ and $\trg{\OB{\alpha_2}}\in\taim{\compaim{\src{\mc{C}_2}}}$.
The algorithm outputs a single \jem component \src{\mc{C}} that is the context that can differentiate between \src{\mc{C}_1} and \src{\mc{C}_2}.
Formally: $\algo{\src{\mc{C}_1},\src{\mc{C}_2},\trg{\OB{\alpha_1}},\trg{\OB{\alpha_2}}}=\src{\mb{C}}$.
The two traces are the same up to the last action, therefore $\trg{\OB{\alpha_1}}\equiv\trg{\OB{\alpha}\alpha_1!}$ and $\trg{\OB{\alpha_2}}\equiv\trg{\OB{\alpha}\alpha_2!}$ where $\trg{\alpha_1!}\neq\trg{\alpha_2!}$.
Trace \trg{\OB{\alpha}} is called the \emph{common prefix} while the two actions $\trg{\alpha_1!}$ and $\trg{\alpha_2!}$ are the \emph{different actions}, which appear at index $i$.

Intuitively, the algorithm produces code \src{\mb{C}} that replicates all ?-decorated actions in the common prefix \trg{\OB{\alpha}}.
The !-decorated actions are made by the component that fills the hole of \src{\mb{C}} and the algorithm adds code to \src{\mc{C}} to update its internal state.
Then, \src{\mb{C}} performs the differentiation by terminating in case it detects \src{\mc{C}_1} and diverging in the other.

The algorithm is divided in three sub-routines: building the skeleton (\skel{\src{\mc{C}_1},\src{\mc{C}_2}}), emulating the common prefix (\emul{\trg{\OB{\alpha}},\trg{t}}) and distinguishing the different actions (\diff{\trg{\alpha_1!},\trg{\alpha_2!},i}).



\paragraph{$\skel{\src{\mc{C}_1},\src{\mc{C}_2}}$}
implements all classes and objects that \src{\mc{C}_1} and \src{\mc{C}_2} specify in their import declarations.
Additionally, it creates helper functions and objects, e.g., it has tables where all globally-known objects are stored and it has a variable to keep track of the action being emulated.








\paragraph{$\emul{\trg{\OB{\alpha}},\trg{t}}$}
returns method bodies that fill the classes created by \skel{\cdot} based on the different encountered actions.
Intuitively, this algorithm subroutine creates a \jem context that emulates all ?-actions in the traces.

\begin{itemize}
	\item$\cl{\trg{a}\ \trg{\OB{w}}}$
	In this case the context must call method \src{m} compiled at address \trg{a}; \trg{t} tells which \aim addresses correspond to which \jem methods.
	Based on the (known) signature of \src{m}, the parameters \trg{\OB{w}} are emulated to their \jem counterpart.
	
	Primitively-typed parameters are emulated to their \jem counterpart.
	For example when a \src{\lstb{Bool}} is expected and \comp{\src{\lst{true}}} is received, the parameter is emulated by \src{\lst{true}}.
	Object-typed parameters are stored in globally-accessible tables based on the encoding of their type and of the id they have in \aim.
	These tables have getters and setters to retrieve objects based on their \aim id.
	
	\item$\rb{\trg{a}\ \trg{w}}$
	In this case the produced code must return the value emulating \trg{w}, as discussed in the call case.

	\item$\cb{\trg{a}\ \trg{\OB{w}}}$ and $\rt{\trg{a}\ \trg{w}}$
	In these cases, the internal state of \src{\mb{C}} is updated.
	For example, \src{\mb{C}} keeps track of the index of the action that is emulating and of all allocated objects.
	In these cases, the index is incremented by 1 and all newly allocated objects received via \trg{\OB{w}} or \trg{w} are added to the tables.
\end{itemize}

There are cases in which a ?-decorated action cannot be emulated, e.g., a return when no method call was made or a call to a method that expects a \src{\lstb{Unit}}-typed parameter and instead receives \comp{\src{\lst{true}}}.
These are actions that try to violate \jem abstractions; in this cases the algorithm must \fail\ and generate a differentiating component that does nothing (\Cref{thm:maintheorem}).
\begin{lemma}[Termination is emulation failure]\label{thm:maintheorem}
$\forall\src{\mc{C}},\comp{\src{\mc{C}}}=(\trg{m_c},\trg{m_d},\trg{t}). \trg{\OB{\alpha}\surd}\in\taim{\compaim{\src{\mc{C}}}} \iff \emul{\trg{\OB{\alpha}},\trg{t}}=\fail$.
\end{lemma}
\Cref{thm:maintheorem} is the most important result of this paper, as proving it reveals which issues arise in a secure compiler.
This \namecref{thm:maintheorem} states that any traces that causes a termination tick cannot be replicated at the source level (i.e., the algorithm \fail s).
An action that cannot be replicated in \jem is an action that tries to violate the abstractions of \jem.
Termination ticks are only generated by the execution of \asm{halt}; only the checks inserted by \prot{\cdot} or by \sys insert that instruction.
Traces with a \trg{\surd} are traces that trigger a check; so they are violating a \jem abstraction in compiled code.
If this is true for all traces with a \trg{\surd} (the $\Rightarrow$ direction), and also all traces that incur violations generate a \trg{\surd} (the $\Leftarrow$ direction) then the algorithm is correct.
Most importantly, this proof indicates where to place the checks at entry points and what to check.
The fact that it is not possible to emulate something (e.g., a \src{\lstb{Bool}}-typed parameter that is not \comp{\src{\lst{true}}} nor \comp{\src{\lst{false}}}) indicates what checks to add (in this case, that \src{\lstb{Bool}}-typed parameters must be either \comp{\src{\lst{true}}} or \comp{\src{\lst{false}}}, i.e., function \fun{dynamicTypechecks}{\cdot}).





\paragraph{$\diff{\trg{\alpha_1!},\trg{\alpha_2!},i}$} 
returns two different code fragments that will detect whether the produced context is interacting with \src{\mc{C}_1} or \src{\mc{C}_2}.
For example, consider the two actions to be $\rt{\trg{a}\ \comp{\src{\lst{true}}}}$ and $\rt{\trg{a}\ \comp{\src{\lst{false}}}}$.
After the last emulated action, the context needs to check the returned value and terminate in case it is \src{\lst{true}} and diverge in the other.

All cases when two !-decorated actions are different are considered in \diff{\cdot}; they are omitted for space reasons.

\medskip

By proving that all of its subroutines are correct, and especially by relying on \Cref{thm:maintheorem}, \algo{\cdot} is proven correct (\Cref{thm:algocorr}).
\begin{theorem}[Algorithm correctness]\label{thm:algocorr}
$\forall\src{\mc{C}_1},\src{\mc{C}_2},\trg{\OB{\alpha}\alpha_1}\in\taim{\compaim{\src{\mc{C}_1}}},\trg{\OB{\alpha}\alpha_2}\in\taim{\compaim{\src{\mc{C}_2}}}, \trg{\alpha_1}\neq\trg{\alpha_2}, |\trg{\OB{\alpha}}|\%2=1, \algo{\src{\mc{C}_1},\src{\mc{C}_2},\trg{\OB{\alpha}\alpha_1},\trg{\OB{\alpha}\alpha_2}}=\src{\mb{C}}\ldotp \src{\mb{C}}[\src{\mc{C}_1}]\divrjem\niff\src{\mb{C}}[\src{\mc{C}_2}]\divrjem$.
\end{theorem}







\subsection{Proofs}\label{sec:allproofs}
By the theorems of \Cref{sec:compcorrdir,sec:compsecdir}, \compaim{\cdot} is fully-abstract (\Cref{thm:compaimisfa}).
\begin{theorem}[\compaim{\cdot} is fully-abstract]\label{thm:compaimisfa}
$\forall\src{\mc{C}_1},\src{\mc{C}_2}.\src{\mc{C}_1}\ceqjem\src{\mc{C}_2}\iff\compaim{\src{\mc{C}_1}}\ceqaim\compaim{\src{\mc{C}_2}}$.
\end{theorem}

The novel result we are after for \compaim{\cdot} is modularity, i.e. components can be compiled separately and linked together afterwards without compromising security.
Indicate the linking of two \aim components \trg{P_1} and \trg{P_2} as $\mylink{\trg{P_1},\trg{P_2}}$.
We want to link any two \aim components \compaim{\src{\mc{C}_1}} and \compaim{\src{\mc{C}_2}} and be sure that $\mylink{\compaim{\src{\mc{C}_1}},\compaim{\src{\mc{C}_2}}}$ is still fully-abstract.
Formally, we have that \Cref{thm:compaimhorizcomp} is a corollary of \Cref{thm:compaimisfa}.
\begin{corollary}[Modular full-abstraction]\label{thm:compaimhorizcomp}
$\forall\src{\mc{C}_1},\src{\mc{C}_2},\src{\mc{C}}.$ $\src{\mc{C}_1;C}\ceqjem\src{\mc{C}_2;C}\iff$ $\mylink{\compaim{\src{\mc{C}_1}},\compaim{\src{\mc{C}}}}\ceqaim\mylink{\compaim{\src{\mc{C}_2}},\compaim{\src{\mc{C}}}}$.
\end{corollary}


==> bodies2/cmds.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%							COMMANDS						  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	TODO annotations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\MP}[1]{\todo[color=blue!30]{TODO: #1}}
\newcommand{\DD}[1]{\todo[color=green!30]{TODO: #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Math formatting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mi}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\mr}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\mt}[1]{\ensuremath{\texttt{#1}}}
\newcommand{\mtt}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\mf}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mk}[1]{\ensuremath{\mathfrak{#1}}}
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\ms}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\mb}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\msc}[1]{\ensuremath{\mathscr{#1}}}

\newcommand{\isdef}{\ensuremath{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily def}}}{=}}}}

% http://tex.stackexchange.com/questions/5502/how-to-get-a-mid-binary-relation-that-grows
\newcommand{\relmiddle}[1]{\mathrel{}\middle#1\mathrel{}}

\DeclareMathOperator\mydefsym{\ensuremath{\iangleq}}
\newcommand\bnfdef{\ensuremath{\mathrel{::=}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Math shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\OB}[1]{\ensuremath{\overline{#1}}}
\newcommand{\llb}{\llbracket}
\newcommand{\rrb}{\rrbracket}
\newcommand{\lla}{\mathopen{\ll}}
\newcommand{\rra}{\mathclose{\gg}}
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\Da}[1]{\ensuremath{\Downarrow^{#1}}}
\newcommand{\Ua}[1]{\ensuremath{\Downarrow^{#1}}}

\newcommand{\myset}[2]{\ensuremath{\{#1 ~|~ #2\}}}
\newcommand{\partof}[1]{\ensuremath{\mc{P}(#1)}}

\newcommand{\compstatus}[0]{\ensuremath{\mc{CS}}}
\newcommand{\compending}[0]{\ensuremath{\mc{CE}}}

\newcommand{\divr}[0]{\ensuremath{\!\!\Uparrow}\xspace}
\newcommand{\term}[0]{\ensuremath{\!\!\Downarrow}\xspace}
\newcommand{\divrjem}[0]{\ensuremath{\src{\Uparrow}}\xspace}
\newcommand{\divraim}[0]{\ensuremath{\trg{\Uparrow}}\xspace}
\newcommand{\termjem}[0]{\ensuremath{\src{\Downarrow}}\xspace}
\newcommand{\probf}[1]{\fun{Pr}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Math environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}%

\AtEndEnvironment{problem}{\null\hfill\QEDA}
\AtEndEnvironment{example}{\null\hfill$\boxdot$}
\AtEndEnvironment{proof}{}%\null\hfill\qed}

\Crefname{lstlisting}{Listing}{Listings}
\Crefname{problem}{Problem}{Problems}

\newenvironment{proofsketch}{\trivlist\item[]\emph{Proof Sketch}.\xspace}{\unskip\nobreak\hskip 1em plus 1fil\nobreak$\Box$\parfillskip=0pt\endtrivlist}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Compiler 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\compskel}[3]{\ensuremath{\bl{\llbracket} #1 \bl{\rrbracket}^{\bl{#2}}_{\bl{#3}}}}
\newcommand{\comp}[1]{\ensuremath{ \bl{(\!|}#1\bl{|\!)} }}
\newcommand{\compgen}[1]{\compskel{#1}{\mc{S}}{\mc{T}}}
\newcommand{\compaim}[1]{\compskel{#1}{\jem}{\aim}}

\newcommand{\funname}[1]{\mtt{#1}}
\newcommand{\fun}[2]{\ensuremath{{\bl{\funname{#1}(}#2{\bl{)}}}}\xspace}
\newcommand{\dom}[1]{\fun{dom}{#1}}

\newcommand{\protname}[0]{protect}
\newcommand{\prot}[1]{\fun{\protname}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Language shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\lc}[0]{\ensuremath{\lambda}-calculus\xspace}
\newcommand{\jjr}[0]{Java Jr.\xspace}

\newcommand{\jem}[0]{\ms{J}{\scriptsize\ms{EM}}\xspace}
\newcommand{\aim}[0]{\ms{A}{\scriptsize\ms{IL}}\xspace}
\newcommand{\ail}[0]{\aim}
\newcommand{\ai}[0]{\ms{A}\texttt{+}\ms{I}\xspace}

\newcommand{\sys}[0]{\compaim{\src{Sys}}\xspace}

\newcommand{\Mmachine}[0]{\ensuremath{\mbox{M-machine}}\xspace}
\newcommand{\Cheri}[0]{\ensuremath{\mbox{Cheri}}\xspace}
\newcommand{\Capsicum}[0]{\ensuremath{\mbox{Capsicum}}\xspace}
\newcommand{\PMA}[0]{\mi{PMA}\xspace}

\newcommand{\ASLR}[0]{ASLR\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Language formatting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\stlccol}[0]{ForestGreen}
\newcommand{\ulccol}[0]{WildStrawberry}
\newcommand{\neutcol}[0]{black}

\newcommand{\col}[2]{\ensuremath{{\color{#1}{#2}}}}
\newcommand{\src}[1]{\col{\stlccol}{{#1}}}		
\newcommand{\trg}[1]{\col{\ulccol }{{#1}}}		

\newcommand{\bl}[1]{\ensuremath{{\col{\neutcol}{#1}}}}

\newcommand{\red}[0]{\ensuremath{\hookrightarrow}}

\newcommand{\fail}[0]{\mi{fail}}
\newcommand{\retback}[0]{\mi{retBack}}
\newcommand{\throw}[0]{\mi{throw}}
\newcommand{\entry}[0]{\mi{entry}}

\newcommand{\secu}[0]{\mi{sec}\xspace}
\newcommand{\inse}[0]{\mi{ins}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Logical relations formatting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\logrelgen}[1]{\ensuremath{\operatorname{\approx}^{#1}}}
\DeclareMathOperator\logrel{\logrelgen{}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Type rules
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{typerule}
\crefname{typerule}{rule}{rules}

\newcommand{\typeruleInt}[5]{%									    % #1 is the title, #2 is the hypotheses. #3 is the thesis, #4 is the label for referencing
	\def\thetyperule{#1}%
	\refstepcounter{typerule}%
	\label{tr:#4}%
	%\ensuremath{\begin{array}{c}\textsf{\scriptsize ({#1})} \\#2 \\\hline{\ensuremath{#3}}\end{array}} \inference
  \ensuremath{\begin{array}{c}#5 \inference{#2}{#3}\end{array}} 
}
\newcommand{\typerule}[4]{%									        % #1 is the title, #2 is the hypotheses. #3 is the thesis, #4 is the label for referencing
  \typeruleInt{#1}{#2}{#3}{#4}{\textsf{\scriptsize ({#1})} \\      }
}
\newcommand{\typerulenolabel}[4]{%									% #1 is the title, #2 is the hypotheses. #3 is the thesis, #4 is the label for referencing
  \typeruleInt{#1}{#2}{#3}{#4}{}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Figures, tables and tikz
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclarelayer{background}
\pgfdeclarelayer{veryback}
\pgfdeclarelayer{veryback2}
\pgfdeclarelayer{veryback3}
\pgfdeclarelayer{back2}
\pgfdeclarelayer{foreground}
\pgfsetlayers{veryback3,veryback2,veryback,background,back2,main,foreground}

\newcommand{\tikzpic}[1]{
\begin{tikzpicture}[shorten >=1pt,auto,node distance=6mm]
\tikzstyle{state} =[fill=white,minimum size=4pt]
\tikzstyle{field} =[fill=gray!5,draw=black!70, rectangle, minimum width={width("whiskersfieldww")+2pt}]]
#1
\end{tikzpicture}
}

\newcommand{\tikzpicT}[1]{
\begin{tikzpicture}[shorten >=1pt,node distance=12mm,auto]
\tikzstyle{state} =[fill=white,minimum size=4pt]
#1
\end{tikzpicture}
}

\newcommand{\myfig}[3]{\begin{figure} [!h]
#1
\vspace{-2em}
\caption{\label{fig:#2}#3}
\end{figure}}

\newcommand{\mytab}[3]{\begin{table} [!h]
\centering \small
#1

\caption{\label{tab:#2}#3}
\end{table}}

\newcommand{\mytabnocap}[1]{\begin{table}[!h]
\centering \small
#1
\end{table}}


\newcommand{\myfigonecol}[3]{\begin{figure*}
#1 
\caption{#3}
\label{fig:#2}
\end{figure*}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Misc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\etal}[0]{\textit{et al.}\xspace} 

\def\botrule{\vspace{-1mm}\hrule\vspace{1mm}}

\newcommand{\link}[1]{\href{#1}{#1}}

\newcommand{\comm}[1]{}

\newcommand{\longcol}[0]{0.3}
\newcommand{\shortcol}[0]{0.11}
\newcommand{\colleng}[0]{0.49}
\newcommand{\fcol}[0]{0.2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\algo}[1]{\ensuremath{\langle\!\langle#1\rangle\!\rangle}}
\newcommand{\skel}[1]{\fun{skeleton}{#1}}
\newcommand{\emul}[1]{\fun{emulate}{#1}}
\newcommand{\diff}[1]{\fun{diff}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% traces
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\traces}[2]{\ensuremath{\ms{Traces}_{#2}(#1)}}
\newcommand{\taim}[1]{\traces{#1}{\aim}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Assembly
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hl}[1]{\color{red!60}{#1}} 
\newcounter{line}

\newcommand{\assline}[1]{\trg{\arabic{line}}~~ \trg{\mtt{#1}}\stepcounter{line}}
\newcommand{\asm}[1]{\trg{\mtt{#1}}}

\newcommand{\xto}[1]{\ensuremath{\xrightarrow{~#1~}}}
\newcommand{\Xto}[1]{\ensuremath{\xRightarrow{~#1~}}}
\newcommand{\xtol}[1]{\ensuremath{\xrightarrow{~#1~}\low}}
\newcommand{\Xtol}[1]{\ensuremath{\xRightarrow{~#1~}\Low}}
\newcommand{\tol}[0]{\ensuremath{\to\low}}
\newcommand{\low}[0]{\ensuremath{\!\!\!\!\to} }
\newcommand{\Low}[0]{\ensuremath{\!\!\!\!\Rightarrow} }
\newcommand{\sst}[0]{\ensuremath{\searrow^{\ms{SS}}}}
\newcommand{\acp}[1]{\ms{#1}}
\newcommand{\blk}[0]{\ensuremath{(\unk,\trg{m},\trg{\OB{s}},\trg{h},\trg{t})}\xspace}
\newcommand{\unk}[0]{\ensuremath{\ms{unk}}}
\newcommand{\unp}[0]{\ensuremath{\mi{un}}}
\newcommand{\stu}[0]{\ensuremath{^{\bot}\xspace}}
\newcommand{\id}[0]{\mi{id}}
\newcommand{\tolai}[0]{\ensuremath{\to}}
\newcommand{\tolaii}[0]{\ensuremath{\tolai^{\!\!\!\!\!i}\ }}
\newcommand{\tolaie}[0]{\ensuremath{\tolai^{\!\!\!\!\!e}\ }}
\newcommand{\toid}[0]{\ensuremath{\xto{\trg{\id}}}}
\newcommand{\tolid}[0]{\ensuremath{\xtol{\trg{\id}}}}
\newcommand{\tolun}[0]{\ensuremath{\xto{\unp}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Listings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\newcommand{\lstb}[1]{\ensuremath{\text{\texttt{\textbf{#1}}}}}
\newcommand{\lst}[1]{\ensuremath{\text{\texttt{{#1}}}}}

\lstdefinelanguage{Java} %thanks to whoever did this
{morekeywords={abstract, all, and, as, assert, but, check, disj, else, exactly, extends, fact, for, fun, iden, if, iff, implies, in, Int, int, let, lone, module, no, none, not, one, open, or, part, pred, run, seq, set, sig, some, sum, then, univ, package, class, public, private, null, return, new, interface, extern, object, implements, System, static, super, try , catch, throw, throws, Unit, var, val, of, principal, trust},
sensitive=true,
%commentstyle=\color{mygreen},
%morecomment=[l][\small\itshape\color{mygreen}]{--},
%morecomment=[l][\small\itshape\color{mygreen}]{//},
%morecomment=[s][\small\itshape\color{mygreen}]{/*}{*/},
%keywordstyle=\color{blue!60!black}\bfseries,
%stringstyle=\ttfamily\color{red!50!brown},
%identifierstyle=\color{purple!40!black},
keywordstyle=\bfseries\color{green!40!black},
commentstyle=\itshape\color{purple!40!black},
morecomment=[l][\small\itshape\color{purple!40!black}]{//},
identifierstyle=\color{blue},
stringstyle=\color{orange},
basicstyle=\small,
basicstyle={\small\ttfamily},
numbers=left,
numberstyle=\tiny\color{mygray},
tabsize=2,
numbersep=3pt,
breaklines=true,
lineskip=-2pt,
stepnumber=1,
captionpos=b,
breaklines=true,
breakatwhitespace=false,
showspaces=false,
showtabs=false,
float=!h,
%frame=single,
columns=fullflexible,escapeinside={(*@}{@*)},
moredelim=**[is][\color{red!60}]{@}{@},
literate={->}{{$\to$}}1 {^}{{$\mspace{-3mu}\widehat{\quad}\mspace{-3mu}$}}1
{<}{$<$ }2 {>}{$>$ }2 {>=}{$\geq$ }2 {=<}{$\leq$ }2
{<:}{{$<\mspace{-3mu}:$}}2 {:>}{{$:\mspace{-3mu}>$}}2
{=>}{{$\Rightarrow$ }}2 {+}{$+$ }2 {++}{{$+\mspace{-8mu}+$ }}2
{<=>}{{$\Leftrightarrow$ }}2 {+}{$+$ }2 {++}{{$+\mspace{-8mu}+$ }}2
{\~}{{$\mspace{-3mu}\widetilde{\quad}\mspace{-3mu}$}}1
{!=}{$\neq$ }2 {*}{${}^{\ast}$}1 %{.}{$\cdot$}1
{\#}{$\#$}1
}
\lstset{language=Java,numbersep=5pt,frame=single}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Contextual equivalence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator\niff{\ensuremath{\mathrel{\iff\!\!\!\!\!\!\!\!\!\!/\ \ }}}
\DeclareMathOperator\nsimeq{\ensuremath{\mathrel{\not\simeq}}}
\DeclareMathOperator\nequiv{\ensuremath{\mathrel{\not\equiv}}}

\DeclareMathOperator\ceq{\ensuremath{\mathrel{\simeq_{\mi{ctx}}}}}
\DeclareMathOperator\nceq{\mathrel{\nsimeq_{\mi{ctx}}}}

\DeclareMathOperator\ceqs{\ceq^\mc{S}}                                       %%
\DeclareMathOperator\ceqt{\ceq^\mc{T}}                                       %%

\DeclareMathOperator\ceqjem{\src{\ceq}}                                      %%
\DeclareMathOperator\nceqjem{\src{\nceq}}                                    %%

\DeclareMathOperator\ceqaims{\trg{\ceq^{\trg{\pi}}}}                 %%
\DeclareMathOperator\nceqaims{\trg{\nceq}^{\trg{\pi}}}               %%
\DeclareMathOperator\ceqaim{\trg{\ceq}}
\DeclareMathOperator\nceqaim{\trg{\nceq}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Trace equivalence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\teqaux#1{\vcenter{\hbox{\ooalign{\hfil
       \raise6pt \hbox{\scriptsize{T}}\hfil\cr\hfil
       $=$}}}}
\def\teqa{\mathrel{\mathpalette\teqaux{}}}
\def\nteqa{\mathrel{\mathpalette\teqaux{}\!\!\!/\ }}

\DeclareMathOperator\teqaims{\ensuremath{\trg{\teqa^{\trg{\pi}}}}}       %%
\DeclareMathOperator\nteqaims{\ensuremath{\trg{\nteqa}^{\trg{\pi}}}}     %%

\DeclareMathOperator\teqaim{\ensuremath{\trg{\teqa}}}       %%
\DeclareMathOperator\nteqaim{\ensuremath{\trg{\nteqa}}}     %%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Well-behaved ceq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ceqwaux#1{\vcenter{\hbox{\ooalign{\hfil
       \raise6pt \hbox{\scriptsize{w-b}}\hfil\cr\hfil
       $\ceq$}}}}
\def\ceqwf{\mathrel{\mathpalette\ceqwaux{}}}
\DeclareMathOperator\ceqw{\ceqwf}
\DeclareMathOperator\ceqwt{\trg{\ceqw}^{\aim}_{\jem}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pre-eq for AIM
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\praux#1{\vcenter{\hbox{\ooalign{\hfil
       \raise6pt \hbox{$\sqsubset$}\hfil\cr\hfil
       $\sim$}}}}
\def\pr{\mathrel{\mathpalette\praux{}}}
\DeclareMathOperator\preqaims{\trg{\pr}^{\trg{\pi}}}
\DeclareMathOperator\preqaim{\trg{\pr}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Traces
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\labelfont}[1]{\ensuremath{\asm{#1}}}
\newcommand{\cl}[1]{\ensuremath{\labelfont{call}\ #1\trg{?}}}
\newcommand{\cb}[1]{\ensuremath{\labelfont{call}\ #1\trg{!}}}
\newcommand{\rt}[1]{\ensuremath{\labelfont{ret}\ #1\trg{!}}}
\newcommand{\rb}[1]{\ensuremath{\labelfont{ret}\ #1\trg{?}}}

\newcommand{\rdl}[1]{\ensuremath{\labelfont{read}#1}}
\newcommand{\wrl}[1]{\ensuremath{\labelfont{write}#1}}

\newcommand{\clgen}[0]{\ensuremath{\labelfont{call}}}
\newcommand{\rtgen}[0]{\ensuremath{\labelfont{ret}}}



\newcommand{\myparagraph}[1]{ \smallskip \noindent\noindent\textit{#1}~}
\DeclareMathOperator\compat{\ensuremath{\raisebox{1mm}{$\frown$}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Missing envs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{conjecture}{Conjecture}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}

\newtheorem{assumption}{Assumption}
\newtheorem{notation}{Notation}
\newtheorem{problem}{Problem}
\Crefname{assumption}{Assumption}{Assumption}
\crefname{assumption}{Assumption}{Assumption}

\theoremstyle{definition}
\newtheorem{definition}{Definition}





\newcommand{\mylink}[1]{\ensuremath{\fun{link}{#1}}}


==> bodies2/intro.tex <==
% !TEX root = ./../scmp.tex
\begin{center}\small
This paper uses colours to distinguish elements of different languages; please print this in colour.
\end{center}


\section{Introduction}\label{sec:intro} 
% context: what is a compiler, what is horizontal compositionality, what is compiler security, what is a component
A compiler is a tool that, among other things, translates programs written in a source language into programs written in a target language.
A compiler is \emph{secure} when it preserves all security properties of the components (i.e., partial programs) it inputs in the components it outputs.
Secure compilation studies compilers that generate target-level components that are as secure as their source-level counterparts.
Full abstraction is the most widely-adopted property to prove when defining a secure compiler~\cite{abadiFa,abadiLayout,Jagadeesan,scoo-j,AhmedFa,ahmedCPS,fstar2js,scoojoin,bugliesi,popldomi,nonintfree}.
A fully-abstract compiler preserves and reflects observational equivalence between the source components it inputs and the target components it produces.
Observational equivalence captures security properties such confidentiality, integrity, etc, and since a fully-abstract compiler preserves all of them, it is a secure compiler.

A compiler is \emph{modular} when it operates on components and its output can be \emph{linked} together into larger components (and possibly into whole programs).

With the advent of machine-code level security architectures (e.g., protected modules architectures (\PMA)~\cite{fidesArch,sancus,intel}, capability machines~\cite{cheri,capsicum}, micro-policies enforcing architectures~\cite{crashsafemachine}, address space layout randomisation~\cite{abadiLayout}, etc.) researchers have investigated secure (fully-abstract) compilation to such architectures~\cite{scoo-j,jannis,abadiLayout,Jagadeesan}.

For secure compilation to \PMA (informally, a low-level memory isolation mechanism), only compilation of a single protected module has been considered. 
Generalizing this to multiple modules, supporting modular compilation and linking of trusted modules at machine code level, would be useful for a number of reasons: (i) code is easier to develop and distribute in standalone components and (ii) merging modules in a single one is not always possible nor desirable.
Concerning (i), standard arguments for separate compilation apply.
Particularly, it is more efficient to compile only the modules that changed and link it against the previously compiled other code as opposed to recompiling the entire code base. 
Moreover, it is common in practice and useful to use libraries that are built from safe source code but only available in compiled form. 
When targeting \PMA with attestation capabilities, a benefit of  having each module in a different protected module is that this makes it possible to attest them independently.
%Concerning (i), when components are developed, a standard argument for efficiency is to compile only the code that has changed and link it against other code as opposed to compiling the entire code base (i.e., when placing all code in a single module).
%Moreover, when components are compiled to \PMA, we foresee that they are distributed in binaries that already provide one (or more) protected modules.
%One benefit of such an approach is that having each module in a different protected module makes it possible to attest them independently.
%In fact, the Intel SGX module attestation primitives work at a single module granularity, and these capabilities are not applicable if all code is to be merged in a single module.
Concerning (ii), there can be several reasons why merging more modules in a single one is not desirable; even with a secure compiler, it can still be useful to protect securely compiled components from each other.
Consider a source language that allows programmers to write both safe and unsafe code at the same time (e.g., Rust, C\# unsafe blocks or the language considered by Juglaret \etal~\cite{catalin}).
A desirable property for a compiler for such a language is that unsafe code does not affect the safe one.
In this case, one can foresee splitting the safe and the unsafe program parts in two different modules and using the secure compiler presented in this paper for the safe part.
In this way, both the safe and the unsafe code cannot be directly violated by an attacker and the unsafe code can not affect the safe one.
Another setting where merging multiple modules is undesirable is when a programmer provides a hand-optimised securely-compiled component that performs better than the ones obtained by a secure compiler, but with the same security guarantees.
In this case, merging such a component with other ones in a single module seems undesirable, as the hand-made assembly can be error-prone and maliciously-crafted.
However, by using a modular secure compiler, other components can still interact with the hand-optimised one and no one's security can be violated.

%A single program can consist of trusted and untrusted parts where the untrusted still must not leak.
%These untrusted parts can be inherent in the programming language (as Juglaret \etal do) or they could derive from hand-optimised code.

% why using more than one module % why not all code in just one (so, why is old technique not usable)
% first: why using more than 1 is nice
% then: we could use the old one even if we were to cancel all these benefits, but ... ... .. 


Extending the compiler to support modular compilation is, however, surprisingly complicated for a number of reasons:
\begin{enumerate}
\item\label{pt:probone} with a single protected module, all run-time meta information about the execution that needs to be protected (e.g.,  the call stack, or dynamic type information) can be stored within that single protected module. 
For a modular compiler, that state must be divided over the various protected modules, or -- possibly -- stored in a centralized trusted protected module.

\item\label{pt:probtwo} with a single protected module, object references are either private to the module or public. 
With support for multiple protected modules, object references can also be shared between some modules and still be unknown to other ones. 
This requires a mechanism for protecting object references that is more elaborate than what the existing secure compiler to \PMA uses.
\end{enumerate}

There are several interesting approaches to address these challenges.
This paper investigates how these issues can be addressed constructing a modular fully-abstract compiler for \PMA in the style of Intel SGX~\cite{intel} \emph{without} additional hardware support.
Even if this turns out to be intricate, we believe there is value in this approach, as this kind of hardware support is available on commercially available systems today, whereas more advanced hardware support is only available in research prototypes.

An alternative approach to modular, secure compilation would be to investigate what kind of novel hardware security architectures can help in addressing these challenges. 
This is the approach taken by Juglaret \etal~\cite{jannis} and it can likely lead to a secure compilation scheme. 
An important downside is that it may take a while before such hardware extensions are available in mainstream systems.

The main contribution of this paper is \compaim{\cdot}, a modular and fully-abstract compiler to SGX-like \PMA.
The source language of \compaim{\cdot} is \jem, an object-based imperative language with method calls and dynamic memory allocation.
The target language of \compaim{\cdot} is \aim, untyped assembly language with an explicit linking mechanism extended with \PMA.
\jem, \aim and \PMA are formalised in \Cref{sec:langform}.
Explicitly considering linking between assembly components generates a number of previously-unobserved problems that are presented in \Cref{sec:probs}.
The main contribution of this paper is the formalisation of \compaim{\cdot}, presented in \Cref{sec:seccomp}.
Supporting additional language features is discussed in \Cref{sec:disc}.
The proof sketch of \compaim{\cdot} being fully-abstract and modular is presented in \Cref{sec:proof}.
Finally, \Cref{sec:rw} discusses related work and \Cref{sec:conc} concludes.

